Strategies for simulating time evolution of Hamiltonian lattice field theories

Simulating the time evolution of quantum field theories given some Hamiltonian $H$ requires developing algorithms for implementing the unitary operator e^{-iHt}. A variety of techniques exist that accomplish this task, with the most common technique used so far being Trotterization, which is a special case of the application of a product formula. However, other techniques exist that promise better asymptotic scaling in certain parameters of the theory being simulated, the most efficient of which are based on the concept of block encoding. In this work we study the performance of such algorithms in simulating lattice field theories. We derive and compare the asymptotic gate complexities of several commonly used simulation techniques in application to Hamiltonian Lattice Field Theories. Using the scalar \phi^4 theory as a test, we also perform numerical studies and compare the gate costs required by Product Formulas and Signal Processing based techniques to simulate time evolution. For the latter, we use the the Linear Combination of Unitaries construction augmented with the Quantum Fourier Transform circuit to switch between the field and momentum eigenbases, which leads to immediate order-of-magnitude improvement in the cost of preparing the block encoding. The paper also includes a pedagogical review of utilized techniques, in particular Product Formulas, LCU, Qubitization, QSP, as well as a technique we call HHKL based on its inventors' names.

==> sec_2_alg_review.tex <==
\section{Review of simulation algorithms}
\label{sec:review_alg}

In this section, we review some algorithms commonly used in the literature for simulating the time evolution of generic quantum systems.
%
We will focus on algorithms based on Product Formulas (PFs)~\cite{childs2019nearly,Childs:2019hts} and Quantum Signal Processing (QSP)~\cite{Low:2016sck,Low:2016znh}, both of which can be applied to small and spatially extended systems.
%
We also review the HHKL algorithm~\cite{Haah:2018ekc}, which may serve as a ``nearly-optimal wrapper'' of local evolution operators in geometrically-local system. These algorithms will serve as the building blocks from which we express algorithms for Hamiltonian lattice field theories in later chapters.

The discussion in this section aims to be a standalone discussion that gives the reader a basic understanding of the different tools used to implement a time evolution operator.
%
While we aim to make this section accessible to readers without much background in the topic, we will still provide a precise set of statements and theorems that will be used later.
%
Note that this section is not detailed enough to re-derive all of these results, and for this we refer the reader to the papers cited in this section.

Note also that this discussion is kept very general, without restricting ourselves to the Hamiltonians considered in this work (except when stated explicitly otherwise).

\subsection{Product-formulas}
\label{PF}

We begin by considering a time-independent Hamiltonian 
\begin{align}
    \label{eq:time_ind_H}
    H = \sum_{\gamma=1}^{\Gamma}H_\gamma
\end{align}
comprised of $\Gamma$ summands, such that one can efficiently construct quantum circuits to implement the exponential $\me^{-iH_\gamma t }$ of each summand appearing on the RHS of \cref{eq:time_ind_H}. 
%
The unitary operator (called the time evolution operator for $H$) given by the exponential $\me^{-iHt}$ describes evolution under the full Hamiltonian $H$ for some arbitrary time $t$. 
%
PFs allow us to construct an approximation to the full time evolution operator by decomposing it into a product of exponentials, each involving a single summand. 
%
The general form of a PF (see Ref. ~\cite{Childs:2019hts}) is given by 
%
\begin{equation}
    \label{def:PF}
    \me^{-iHt} \approx
    S(t) = \prod_{\upsilon=1}^{\Upsilon}\mathcal{P}_\upsilon\!\left(\prod_{\gamma = 1}^{\Gamma}\me^{-ita_\upsilon^{(\gamma)}H_{J}}\right)
    ,
\end{equation}
%
such that each $a_\upsilon^{(\gamma)} \in \mathbb{R}$ and $\sum_{\upsilon=1}^{\Upsilon}a_\upsilon^{(\gamma)} = 1$ $\forall \gamma \in [\Gamma] \equiv \{1,2,\dots,\Gamma\}$. 
%
The latter condition ensures that each individual term $H_\gamma$ is evolved for the total time $t$. 
%
The parameter $\Upsilon$ determines the total number of stages in the PF, and for each stage $\upsilon \in [\Upsilon]$ there exists a corresponding permutation operator $\mathcal{P}_\upsilon$ that determines the ordering of the individual exponentials within that stage (the specific actions of the operators $\mathcal{P}_\upsilon$ depend on the chosen PF construction). 
%
PFs of the form \cref{def:PF} provide good approximations to the full time evolution operator when the evolution time t is small, and in particular one defines a $p^{\text{th}}$ order PF $S_p(t)$ as one that is correct up to $p^{\text{th}}$ order in $t$
\begin{align}
\label{eq:pth_order_PF_intro}
    S_p(t) = \me^{-iHt} + \mathcal{O}(t^{p+1})\,.
\end{align}
%
The simplest example of a PF arises from the use of the Baker-Campbell-Hausdorff formula 
%
\begin{align}
    \me^{A+B} = \me^A \me^B + \OO([A,B])
    \,,
\end{align}
%
and thus we can write
%
\begin{align}
    \me^{-iHt} \approx S_1(t) =  \prod_{\gamma=1}^{\Gamma} \me^{-iH_\gamma t }
    \,.
\end{align}
%
This approximation is known as the first order Lie-Trotter formula. The higher (even) order Suzuki-Trotter formulas are defined recursively as
\begin{align}
S_2(t) &\coloneqq \prod_{i=1}^{\nterms}\me^{\frac{-iH_it}{2}}\prod_{i=\nterms}^{1}\me^{\frac{-iH_it}{2}}\,,
    \nonumber\\
    S_{2k}(t) &\coloneqq S_{2k-2}(u_kt)^2S_{2k-2}((1-4u_k)t)\nonumber\\
    & \qquad \qquad \times S_{2k-2}(u_kt)^2\,,
\label{eq:pth_order}
\end{align}
%
where $u_k \equiv 1/\left(4 - 4^{1/(2k-1)}\right)$,  and the product given by $\prod_{i=\nterms}^{1}\left( \cdot \right)$ corresponds to reversing the order in which we choose the variable $i$ with respect to the first product given by $\prod_{i=1}^{\nterms}\left( \cdot \right)$. 
%
In theory, one could use such a construction to build arbitrarily large order PFs. 
%
However the number of stages $\Upsilon$, and hence the number of elementary gate operations required to construct a circuit implementing such a PF, grows exponentially with the order $p$ (see Ref.~\cite{Childs:2019hts}). 
%
For this reason, we use relatively low order formulas for practical applications and our results assume that $p,\Upsilon(p) = \OO(1)$.
%
\CFK{
Note that~\cref{eq:pth_order} is only one possible form of~\cref{def:PF}, and investigating alternatives to it is an active area of research~\cite{Hastings:2014wyq,Poulin:2014yec,tranter2018comparison,Hu:2022nyd,tranter2019ordering,Schmitz:2021ruv,Ostmeyer:2022lxs}.
}

Since PFs have corrections that depend polynomially on the evolution time $t$, they give good approximations for small $t$. Given a PF valid for small $t$, however, we can obtain one for longer times.
%
The general procedure is to divide the full evolution time $t$ into $r$ (known as the \emph{Trotter number}) smaller time steps, and apply the chosen $p^{\text{th}}$ order PF to each step, describing the evolution for a smaller time $t/r$, before multiplying together the results from the individual steps
%
\begin{align}
    S_p(t) = (S_p(t/r))^r,
\end{align}
%
and the associated exponentation error $\varepsilon$ is given by
%
\begin{equation}
\label{eq:exp_error}
    \varepsilon = \|(S_p(t/r))^r - \me^{-iHt }\|
    \,.
\end{equation}
%
To work out the resource requirements to satisfy such an error bound, we ask for the required Trotter number $r$ for a $p^{\text{th}}$ order formula to satisfy \cref{eq:exp_error} given a fixed value of $\varepsilon$. 
%
In general the answer depends on the asymptotic scaling on the evolution time $t$, as well as the norms of the individual summands $H_\gamma$ and the commutators amongst them. 

While \cref{eq:pth_order_PF_intro} provides the correct asymptotic dependence of the error on $t$, Refs.~\cite{Childs:2019hts} and~\cite{Berry:2005yrf} present bounds that show explicit dependence on the 1-norm of the full Hamiltonian (given by $\sum_{\gamma=1}^{\nterms}\|H_\gamma\|$). 
%
Note however, that these bounds are not tight. 
%
For example, when all the summands $H_\gamma$ commute, the exponentiation error $\varepsilon$ becomes zero while these error bounds can become arbitrarily large. 
%
This was further addressed in Ref \cite{Childs:2019hts}, where the authors present another (tighter) bound that results from exploiting the commutativity properties of the summands $H_\gamma$. 
%
This led to the following asymptotic scaling of the Trotter number
\begin{equation}\label{eq:trotter_number_1}
            r = \OO\!\left( \frac{\Tilde{\alpha}^{\frac{1}{p}}t^{1 + \frac{1}{p}}}{\varepsilon^{\frac{1}{p}}} \right)
            \,,
        \end{equation}
where $\Tilde{\alpha} \equiv \sum_{\gamma_1,\gamma_2,...,\gamma_{p+1} = 1}^{\Gamma} \lvert\lvert [ H_{\gamma_{p+1}},... [H_{\gamma_2},H_{\gamma_1}] ] \rvert\rvert$.

Note that not every Trotter number $r$ satisfying the asymptotic upper bound \eqref{eq:trotter_number_1} will yield the desired error bound. Rather, the above result merely provides an asymptotic upper bound on the \textit{minimum} Trotter number $r$ needed.

\subsection{Quantum Signal Processing}
\label{QSP}

While most applications to date simulating relativistic quantum field theories use PFs as discussed in~\cref{PF}, there is an alternate approach for simulating the time evolution of quantum systems that is based on a very general technique called \emph{Quantum Signal Processing} (QSP).
%
There are two main motivations for studying QSP-based quantum simulation algorithms are: First they have a better asymptotic complexity than PFs~\cite{Low:2016sck,Low:2016znh}. Second they are compatible with a wider class of Hamiltonians than those which can be efficiently mapped onto Pauli Hamiltonians, and for which the number of qubits is sublinear in the number of degrees of freedom in the system~\cite{Babbush:2019yrx,Kreshchuk:2020dla,Kirby:2021ajp}.

As with PFs, the aim of this section is a pedagogical overview of techniques based on QSP, however we do provide precise statements of the theorems needed in the rest of the paper. 
%
We will rely on results from the literature to provide proofs of these theorems. 

Simulating the time evolution operator of a given Hamiltonian using QSP relies on a a few key insights, which we will now review in turn.

\subsubsection{Idea of block encoding}
\label{sec:BEidea}

\begin{figure}[h]
\begin{quantikz}
\lstick{$\sket{g}_a$}& \gate[2]{U_A} \qwbundle{}& \meter{} & \setwiretype{c} \rstick{$\sket{g}_a$}\\
\lstick{$\sket{\psi}_s$} & \qwbundle{} \qw & \qw \rstick{$\dfrac{A\sket{\psi}_s}{\|A\sket{\psi}_s\|}$}
\end{quantikz}
\caption{Circuit implementing the block encoding $U_A$ of an operator $A$, as defined in~\cref{eq:BEdef}. If the ancillary register is measured in the state $\sket{g}_a$, the state of the system is ${A\sket{\psi}_s}/{\|A\sket{\psi}_s\|}$.}
\label{fig:BE}
\end{figure}

Block encoding (BE) is a technique that allows one to implement the action of a given operator $A$ on an arbitrary quantum state directly in a quantum circuit, despite this operator not being unitary.
%
This can be accomplished by rescaling $A$ and padding it with extra entries to fit it into a unitary matrix that can act simultaneously on the given quantum state together with an appropriate number of ancilla qubits.
%
Schematically, this means that the operator $A$, which acts on a system Hilbert space ${\cal H}_s$, is embedded into a unitary matrix acting on a larger Hilbert space ${\cal H}_a \otimes {\cal H}_s$, where ${\cal H}_a$ is the Hilbert space of the ancillary qubits. Schematically, $U_A$ is given by
%
\begin{align}
\label{eq:BEdef}
    U_A = 
    \begin{pmatrix}
        A / \alpha & * \\
        * & *
    \end{pmatrix}
    .
\end{align}
%
The rescaling by the parameter $\alpha$, known as \emph{scale factor}, is required, since the norm of any subblock of a unitary matrix has to be less than unity. 
%
\Cref{eq:BEdef} therefore implies that $U_A$ is, in fact, a BE for the entire equivalence class of matrices $A$ differing by a constant factor.

If we define the state $\sket{g}_a$ as the state that projects out the block of $U_A$ containing the operator $A/\alpha$, we can write
\begin{align}
    \label{eq:beproj}
    A/\alpha &= (\sbra{g}_a\otimes \unit_s) U_A (\sket{g}_a\otimes \unit_s) \\
    \sket{g}_a\sket{\psi}_s &=
    \begin{pmatrix}
        \sket{\psi}_s \\ 0
    \end{pmatrix}_a \nonumber\\
    U_A \sket{g}_a\sket{\psi}_s &= 
    \begin{pmatrix}
        A \sket{\psi}_s \\ \ast 
    \end{pmatrix}
    = 
        \sket{g}_a (A \sket{\psi}_s) + \sket{\bot}_{as}\nonumber
        \,,
\end{align}
%
where $\sket{\bot}_{as}$ is a vector perpendicular to $\sket{g}_a$. 
%
This implies that $A$ is only applied to $\sket{\psi}_s$ iff the ancillary register is measured in $\sket{g}_a$. 
%
We shall term the probability of this to happen ``success probability of the block encoding''.


The success probability depends on how exactly $U_A$ is constructed.
%
In order for the algorithm to be considered efficient, the success probability has to scale inverse polynomially with problem parameters.
%
The scale factor plays its role in defining the complexity of the simulation algorithm, as will be discussed later.

In much of this work we will use this technique to block encode a Hamiltonian $H$, and we call the corresponding BE $U_H$.
%
The scale factor can then be absorbed by evolving a rescaled Hamiltonian
%
\begin{align}
    \tilde{H} = H / \alpha\,,
\end{align}
%
for the time
%
\begin{equation}
\tilde{t} = \alpha \, t\,,    
\end{equation}
%
so that
%
\begin{equation}
    Ht = \tilde{H} \tilde{t}\,.
\end{equation}

In the following discussion, we will choose a diagonal basis for the (rescaled) system Hamiltonian, such that basis vectors of the system Hilbert space are eigenstates of the Hamiltonian
%
\begin{align}
    \tilde{H} \sket{\lambda}_s = \lambda \sket{\lambda}_s 
    \,,
\end{align}
with $|\lambda| < 1$.
%
This basis is used only to simplify the discussion of the technique.
%
Being able to diagonalize the Hamiltonian is not required for its use.

As already discussed, the vector $\sket{g}_a$ of the ancillary Hilbert space ${\cal H}_a$ defines the block in which the Hamiltonian is encoded in the unitary matrix $U_H$. 
%
In other words, the BE acts on the tensor product of a state $\sket{\lambda}_s$ and $\sket{g}_a$ as
%
\begin{align}
\label{eq:UHaction}
    U_H \sket{g}_a\sket{\lambda}_s = \lambda\, \sket{g}_a\sket{\lambda}_s + \sqrt{1-\lambda^2} \sket{\bot^\lambda}_{as}
    \,,
\end{align}
%
where we have defined a normalized transverse state that is orthogonal to the vector $\sket{g}_a$, such that $(\sbra{g}_a\otimes \unit_s)\sket{\bot}_{as}=0$.
%
Thus, the action of $\tilde{H}$ can be extracted by acting with $U_H$ on an enlarged Hilbert space and post-selecting on the ancilla qubit being in the $\sket{g}_a$ state, \textit{i.e.}
%
\begin{align}
    \sbra{g}_a U_H \sket{g}_a\sket{\lambda}_s = \lambda\, \sket{\lambda}_s
    \,.
\end{align}
%
Note that if the ancillary Hilbert space ${\cal H}_a$ is 2-dimensional, one could choose $\sket{g}_a = \sket{0}_a$ and $\sket{\bot}_a = \sket{1}_a$. 

Many different techniques for BE have been discussed in the literature. 
%
Among many others, one can use general algorithms such as the FABLE algorithm~\cite{camps2022fable}, approaches that rely on a technique called linear combination of unitaries (LCU)~\cite{Childs:2012gwh,Lin:2022vrd}, a technique called QETU~\cite{Dong:2022mmq}, and techniques using access to the matrix elements of the sparse matrix and compact mappings $H$~\cite{Low:2016znh,Lin:2022vrd,Toloui:2013xab,Babbush:2017oum,Kirby:2021ajp,Kreshchuk:2020dla}.
%
The choice of BE is typically dictated by the number of ancillary qubits required, the value of the scale factor $\alpha$, the gate complexity required for its implementation, whether an approximate implementation of the Hamiltonian is sufficient, and whether it is applicable to general sparse Hamiltonians.

One issue with BEs discussed so far is that the action of the BE does not stay in the Hilbert space spanned by ${\rm span}\{\sket{g}_a \sket{\lambda}_s, \sket{\bot^\lambda}_{as}\}$. 
%
In other words, the action of $U_H$ on $\sket{\bot^\lambda}_{as}$ can produce a state with different value of $\lambda' \neq \lambda$, such that in general
%
\begin{align}
\begin{aligned}
    \sbra{g}_a\sbra{\lambda'}_s U_H \sket{g}_a\sket{\bot^\lambda}_{as} &\neq 0\\
    \sbra{\bot^{\lambda'}}_{as} U_H \sket{\bot^\lambda}_{as} &\neq 0
    \,.
\end{aligned}
\end{align}
%
Therefore, repeated actions of the unitary $U_H$ are not easily known.
%
%
This can be dealt with by constructing a more constrained BE $W_H$, for which one can ensure that multiple actions of this BE on a given eigenstate will never produce a state with a different eigenvalue. 
%
This constrained BE is called a \emph{qubitized block encoding} and is discussed in the following section.

\subsubsection{LCU and other techniques for block encoding}
\label{sec:BEtech}
% \paragraph{\underline{Linear Combination of unitaries (LCU)}}
\begin{figure*}[t]
\begin{quantikz}%[row sep = 0.5cm]
\lstick[4]{$\sket{0^{\otimes k}}_a$}
% \lstick{$\sket{0}$}
& \gate[4]{\PREPARE} & \octrl{1} \gategroup[5,steps=4,style={dashed,rounded corners, inner
sep=6pt}]{$\SELECT$} & \ctrl{1} & \qw \ \cdots \ & \ctrl{1} & \gate[4]{\PREPARE^\dagger} & \meter{} & \setwiretype{c} \rstick{$0$} \\
% \lstick{$\sket{0}$}
& & \octrl{1} & \octrl{1} & \ \cdots \ & \ctrl{1} && \meter{} & \setwiretype{c} \rstick{$0$}\\
% \lstick{$\vdots$}
\vdots \setwiretype{n}& & \ \vdots \  & \vdots & \ \ddots \  \setwiretype{n} & \ \vdots \ && \ \vdots \ & \ \vdots \ \\
% \lstick{$\sket{0}$}
&  & \octrl{1} \wire[u][1]{q} & \octrl{1} \wire[u][1]{q} & \ \cdots \ & \ctrl{1} \wire[u][1]{q} && \meter{} & \setwiretype{c} \rstick{$0$}\\
\lstick{$\sket{\psi}_s$} & \qw \qwbundle{} & \gate{U_0} & \gate{U_1} & \ \cdots \ & 
\gate{U_{M-1}} &&& \rstick{$T\sket{\psi}_s/\|T\sket{\psi}_s\|$}
\end{quantikz}
\caption{Linear Combination of Unitaries (LCU) implements t he BE $U_T$ of an operator $T$ expressed as a sum of elementary operators with known circuit implementations, reproduced from Ref.~\cite{Childs:2012gwh}.
Each operator $U_i$ is controlled on the binary string representing its index $i$.
The size of the ancillary register is $k=\lceil\log_2M\rceil$.
For illustration purposes, $\log_2 (M)$ is assumed to be an integer $k$ such that the binary string of $M-1$ contains all 1's.
}
\label{fig:LCU}
\end{figure*}
We begin this section by reviewing a generic subroutine, Linear Combination of Unitaries (LCU) which, \emph{inter alia}, can be used as a general-purpose technique for constructing BEs of qubit Hamiltonians.
%
Then we briefly discuss several modifications of LCU as well as alternative approaches to constructing BEs.

Consider the situation were one has a combination of $M$ unitary operators $U_0$, \ldots, $U_{M-1}$, each acting on a system Hilbert space ${\cal H}_s$ and the goal is to construct the operator
%
\begin{align}
    \label{eq:lcuT}
    T = \sum_{i=0}^{M-1} \beta_i \, U_i
    \,,
\end{align}
%
acting on the same system Hilbert space.\footnote{We assume $\beta_i>0$ since the complex phases of $\beta_i$ can be absorbed by $U_i$.} 
%
\footnote{This technique can also be used to add non-unitary operators by first block-encoding them and then adding the unitaries using LCU.}

This can be achieved in the following way. 
%
First, consider an ancilla register with Hilbert space ${\cal H}_a$ containing $k = \lceil \log M \rceil$ qubits.
%
Labeling the computational basis of these states through the integers corresponding to the binary string encoded in the qubits, one defines a so-called \PREPARE oracle to create a state $\sket{\beta}$:
%
\begin{align}
    \label{eq:prepstate}
   \sket{\beta}_a = \PREPARE_a \sket{0}_a = \frac{1}{\sqrt\beta} \sum_{i=0}^{M-1} \sqrt{\beta_i} \sket{i}_a
   \,,
\end{align}
where $\sket{0}_a$ corresponds to the state with all qubits in ${\cal H}_a$ in the $\sket{0}_a$ state and we have defined $\beta \equiv \|\vec{\beta}\|_1 = \sum_i |\beta_i|$.

Next, using the so-called $\SELECT$ oracle, one performs operations $U_i$ on states in ${\cal H}_s$, controlled on the values of qubits in ${\cal H}_a$
%
\begin{align}
    \label{eq:lcuselect}
    \SELECT = \sum_{i=0}^{M-1} \sket{i}_a \sbra{i}_a \otimes U_i 
    \,.
\end{align}
%
At the end one reverses the prepare oracle. 
%
The complete circuit on the Hilbert space ${\cal H}_{as} = {\cal H}_{a} \otimes {\cal H}_{s}$ can therefore be written as
\begin{align}
    \label{eq:lcube}
    U_T = (\PREPARE_a^\dagger \otimes \unit_s) \, \SELECT \, (\PREPARE_a \otimes \unit_s) \,.
\end{align}
%
Letting this operator act on a state $\sket{0}_a \sket{\psi}_s$ one finds
\begin{align}
    U_T\sket{0}_a \sket{\psi}_s = \frac{1}{\beta}\sket{0}_a T \sket{\psi}_s + \sket{\bot}_{as}
    \,,
\end{align}
where $\sket{\bot}$ is an unnormalized state transverse to $(\sket{0}_a\otimes \unit_s)$.
%
This implies that $U_T$ is a BE of $T$. 

From the above discussion it is clear that the number of ancilla qubits to combine $M$ unitaries is given by ${\rm dim}({\cal H}_a) \sim \log M$, and the number of gates is given by $M$ gates that are controlled on $\log M$ qubits, which can be reduced to $\OO(M \log M)$ elementary gates.

While the presented approach to LCU relies on the binary encoding of terms on the RHS of~\cref{eq:lcuT} in the ancillary register, other encodings can be used as well.
%
In particular, a variation of the LCU algorithm exists, which takes advantage of the Hamiltonian locality~\cite{Kirby:2022ncy}.
%
For an $k$-local $\nq$-qubit Hamiltonian, it requires $2\nq$ ancillary qubits yet only uses $2k$-controlled gates.

The LCU algorithm can be applied to a Hamiltonian provided in a form of a ${2^{\nq}\times2^{\nq}}$ matrix, upon decomposing it into  Pauli strings as $H=\sum_{i=0}^{4^{\nq}-1} \beta_i P_i$, where $P_i$ are the Pauli strings and the coefficients $c_i$ are found as $c_i=\frac{1}{2^{\nq}}\operatorname{Tr}(H P_i)$.
%
An alternative approach to constructing BEs for Hamiltonians given in the matrix form is considered in Ref.~\cite{camps2022fable}.

The LCU approach is often combined with other methods.
In~\cref{sssec:lcuft,sssec:lcuqetu} we shall consider its modifications which take into account the structure of particular lattice Hamiltonians.

Lastly, we briefly mention that simulation techniques based on BE, considered in the next section, are compatible with a wide class of \emph{sparse} Hamiltonians, including those which cannot be efficiently mapped onto Pauli strings.
%
A general approach to constructing BEs for such systems is based on the usage of \emph{sparse oracle} subroutines.
%
As was mentioned in~\cref{sec:introduction}, their construction is highly problem-specific~\cite{Toloui:2013xab,Babbush:2018ywg,Kreshchuk:2020dla,Kirby:2021ajp,rhodes2024exponential} and does not seem to provide advantage over LCU for local HLFTs ~\cite{rhodes2024exponential}, which are considered the main application of this work.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Qubitization}
A \emph{qubitized block encoding} $W_H$ \MK{(also known as \emph{Szegedy quantum walk operator})[])}\MK{Also we should cite somewhere this~\cite{Babbush:2018ywg} paper as it also has a nice introduction to qubitization, see e.g. eq (9). We will cite this if end up adding Fig. 1 from there.} of the Hamiltonian is a BE which remains in the subspace of ${\rm span}\{\sket{g}_a \sket{\lambda}_s, \sket{\bot^\lambda}_{as}\}$ such that one has
%
\begin{equation}
\begin{aligned}
\label{eq:Whdef}
W_H \sket{g}_a\sket{\lambda}_s &= \lambda\, \sket{g}_a\sket{\lambda}_s - \sqrt{1-\lambda^2} \sket{\bot^\lambda}_{as} \\
    &= \left( \lambda\, \sket{g}_a - \sqrt{1-\lambda^2} \sket{\bot^\lambda}_a
 \right)\sket{\lambda}_s
    \,,    
\end{aligned}    
\end{equation}
%
where we have defined
% $\sket{\bot^\lambda}_a$ through 
$\sket{\bot^\lambda}_{as} \equiv \sket{\bot^\lambda}_a \sket{\lambda}_s$  for all eigenstates $\sket{\lambda}$.
%
Note that the minus sign between the two terms is conventional.
%
\CFK{Using the Gram–Schmidt process,} the orthogonal state $\sket{\bot^\lambda}_a$ can now be defined as
%
\begin{align}
\sket{\bot^\lambda}_a\sket{\lambda}_s = \frac{\lambda \unit_{as} - W_H  }{\sqrt{1-\lambda^2}}\sket{g}_a\sket{\lambda}_s
    \,.
\end{align}
%
This works for any dimension of the ancilla Hilbert space ${\cal H}_a$, and implies that for each eigenvalue $\lambda$ of the Hamiltonian there is one specific transverse vector in ${\cal H}_a$. 

\MK{Christian, we significantly revised the notations in the next few equations.}

%\Cref{eq:Whdef} 
Equation~\ref{eq:Whdef} implies the operator $W_H$ is block diagonal, and can be written as
%
\begin{align}
    \label{eq:wwtilde}
    \left(\unit_a \otimes \sbra{\lambda'}_s\right) W_H \left(\unit_a \otimes \sket{\lambda}_s\right) = \widetilde{W}_H^{(\lambda)} \delta_{\lambda \lambda'}
    \,,
\end{align}
where $\widetilde{W}_H^{(\lambda)}$ is some operator acting on the register $a$.
%
Information relevant to block encoding of $H$ is contained in two-dimensional blocks of $\widetilde{W}_H^{(\lambda)}$ corresponding to subspaces
\begin{equation}
h_{a}^{(\lambda)}={\rm span}\{\sket{g}_a, \sket{\bot^\lambda}_{a}\} \in {\cal H}_a \,,
\end{equation}
which we denote by $W_H^{(\lambda)}$:
%
% with $W_H^{(\lambda)}$ acting on the two-dimensional Hilbert space  ${\rm span}\{\sket{g}_a, \sket{\bot^\lambda}_{a}\} \in {\cal H}_a$
%
\begin{align}
\label{eq:wwtildematrix}
\begin{aligned}
W_H^{(\lambda)} &= \begin{pmatrix} \sbra{g}_a \widetilde{W}_H^{(\lambda)} \sket{g}_a & \sbra{g}_a \widetilde{W}_H^{(\lambda)} \sket{\bot^\lambda}_a \\  \sbra{\bot^\lambda}_a  \widetilde{W}_H^{(\lambda)} \sket{g}_a & \sbra{\bot^\lambda}_a  \widetilde{W}_H^{(\lambda)} \sket{\bot^\lambda}_a \end{pmatrix}_{h_{a}^{(\lambda)}}
    \\
    &= \begin{pmatrix} \lambda & - \sqrt{1-\lambda^2} \\ \sqrt{1-\lambda^2} & \lambda \end{pmatrix}_{h_{a}^{(\lambda)}}
    \\
    &= \exp ( -i Y \theta_\lambda)
    \,,    
\end{aligned}
\end{align}
where 
% $Y_{a^{(\lambda)}}$ is the Pauli-$Y$ operator acting on the subspace $h_{a}^{(\lambda)}$, and
\begin{align}
    \theta_\lambda = \arccos(\lambda) \,.
\end{align}
%
While so far we have only defined the unitary $W_H$ through its action on a given state, a very important result is that it can be obtained from a BE of the Hamiltonian $U_H$ using a process known as \emph{qubitization}~\cite{Low:2016znh}, which we now describe.

\CFK{changes start here}
% \MK{plz optimize}
% In many cases of interest, one can seek for $W_H$ in the form of $W_H = S' U_H$ for some operator $S'$ acting solely on ancillary qubits.

In many cases of interest, it is possible to construct the iterate by assuming a form $W_H = S' U_H$, and searching for some $S'$ that acts only on the ancillary qubits. 
The conditions $S'$ must satisfy can be stated more succinctly by first letting $S'$ be a product of a reflector $R_{a}$ about the state $\sket{g}_a$ and another operator $S = S_a \otimes \unit_s$ that acts only on the ancillary qubits, \emph{i.e.}
%
\begin{equation}
\label{eq:Whdefas}
    W_H = \left(R_a \otimes \unit_s \right) \left( S_a \otimes \unit_s \right) U_H\,,
\end{equation}
%
where 
%
\begin{equation}
    R_a = \left(2 \sket{g}_a \sbra{g}_a - \unit_a \right).
\end{equation}
%
Written in this way, it was shown~\cite{Low:2016znh} that one can construct $W_H$ from \Cref{eq:Whdefas} if $S$ satisfies
%
\begin{align}
    \left(\sbra{g}_a \otimes \unit_s \right) S U_H \left(\sket{g}_a \otimes \unit_s \right) &= H,
    \\
    \left(\sbra{g}_a \otimes \unit_s \right) S U_H S U_H \left(\sket{g}_a \otimes \unit_s \right) &= \unit_a\,.
\end{align}

One particularly simple case is when when $U_H$ is its own inverse, \emph{i.e.} $U_H^2 = \unit_{as}$.
In this case, one can simply set $S = \unit_{as}$.
This construction can be applied to the case when the block encoding $U_H$ is constructed via the LCU procedure~\cite{Babbush:2018ywg}. 
To see this, we must modify our perspective slightly.
In the original construction, we had $U_H = (\PREPARE^\dagger) \SELECT (\PREPARE)$ and $\sket{g}_a = \ket{0}_a$.
In this modified perspective, we regroup terms and instead take $U_H \to U_H^\text{LCU} \equiv \SELECT$ and $\sket{g}_a \to \sket{g^\text{LCU}}_a \equiv \PREPARE \sket{0}_a$.
\CFK{could add an equation to make totally explicit, what do people think?}
Because $(U_H^\text{LCU})^2 = \SELECT^2 = \unit_{as}$, we can simply set $S = \unit_{as}$ to construct $W_H$.


% \MK{The construction above can be applied to the case when the block encoding $U_H$ is constructed via the LCU procedure. 
% To see that, instead of ...
% $U_H = \PREPARE^\dagger \SELECT \PREPARE$, let's take the perspective that 
% $\sket{g}\equiv\PREPARE\sket{0}$ and $U_H = \SELECT$. In this way, $S=1$... satisfies above becaues $\SELECT^2 = 1$}
%
% An example of finding $S'$ for the QETU algorithm in considered in \Cref{}.
%

If one uses a method other than LCU to construct $U_H$, a dedicated study must be performed to find $S$.
Since $S$ acts only non-trivially on the ancillary register, this a difficult task in general.
This difficulty can always be overcome, however, by introducing a single ancillary qubit and performing two controlled calls to $U_H$~\cite{Low:2016znh}.
Note that while this procedure does not increase the asymptotic cost of preparing $W_H$, it does result in a significant increase of the overall prefactor. 
%For the methods of constructing $U_H$ in this work, the operators $S$ are known and we can therefore avoid this extra cost. 
Importantly, for all methods used in this work, the operator $S$ is known or was determined, and the expensive general procedure was avoided.
%For all methods used in this paper, the operator $S$ was determined and we therefore avoided the costly implementation of the general case.
For completeness, the general procedure for constructing $W_H$ from an arbitrary $U_H$ can be found in App.~\ref{app:general_W}.
% \CFK{For LCU, take perspective that $U_H \to \SELECT$, for QETU simply say $S = Z$.}
\CFK{in progress}

\CFK{everything below this (in this section) is old, I am re-writing to include discussion about $S$, etc.}
While so far we have only defined the unitary $W_H$ through its action on a given state, a very important result is that it can be obtained from a general (not qubitized \CFK{actually, I think the procedure for constructing $W_H$ from a general BE $U_H$ is precisely referred to as qubitization...}) BE $U_H$.
%
\CFK{move all discussion about qubitization and the $q$ register to appendix. mention here this $S$ operator, and that for LCU or QETU we know it}
The basic idea is to construct orthogonal subspaces using a Gram-Schmidt procedure, and then implementing this through appropriate basis rotations. 
%
This construction requires adding one qubit $\sket{q}$ to the ancillary Hilbert space, such that ${\cal H}_a \to {\cal  H}_{qa} = {\cal H}_q \otimes {\cal H}_a$.
In this new ancillary Hilbert space we define
%
\begin{align}
    \sket{g}_{qa} = \sket{+}_q \sket{g}_a
    \,,
\end{align}
and the operator $W_H$ is defined on the Hilbert space ${\cal H}_{qas} = {\cal H}_q \otimes {\cal H}_a \otimes {\cal H}_s$. 
\begin{figure}[h]
\begin{quantikz}
\lstick{$\sket{}_q$}    & \gate{\Hgate}          
& \octrl{1} \gategroup[3,steps=2,style={dashed, rounded corners,inner sep=6pt},label style={label position=below,anchor=north}]{$\vphantom{\biggl(}U'_{qas}$}        & \ctrl{1}  & \gate{\Xgate} & \gate[2]{R_{qa}} & \gate{\Hgate} & \qw \\
\lstick{$\sket{}_a$}  & \qw \qwbundle{}
& \gate[2]{U_H^{\phantom{\dagger}}} & \gate[2]{U_H^\dagger} & \qw & \qw & \qw & \qw\\
\lstick{$\sket{}_s$} &\qw\qwbundle{}  
&  &  & \qw     &\qw & \qw & \qw 
\end{quantikz}
\caption{
Circuit for the qubitized block encoding $W_H$, given an arbitrary block encoding $U_H$. The circuit for $R_{qa}$ is shown in~\cref{fig:R}.
}
\label{fig:BEW}
\end{figure}
%
\begin{figure}[h]
\begin{quantikz}
\lstick{$\sket{}_q$} & \gate{\Hgate} & \qw & \octrl{1} & \qw & \gate{\Hgate} & \gate{-1} &\\
\lstick[4]{$\sket{}_a$} & \gate[4]{G^\dagger} & & \octrl{1} & & \gate[4]{G} & \qw & \\
\vdots \ \setwiretype{n} &  & & \ \vdots \ & & & \vdots & \\
& & & \octrl{1} \wire[u][1]{q} & & & \qw & \\
& & \gate{\Xgate} & \gate{\Zgate} & \gate{\Xgate} & & \qw &
\end{quantikz}
\caption{
Circuit for the reflection operator $R_{qa}$ defined in~\cref{eq:refl} and used in~\cref{eq:Whdefqas}, see Ref~\cite{Lin:2022vrd} for alternative implementations. $G$ is the oracle for preparing the state $\sket{g}_a$, i.e. ${G\sket{0}_a=\sket{g}_a}$.
The $\boxed{-1}$ gate adds an overall phase to the circuit (negative sign), and can be implemented, e.g., as $\Xgate\Zgate\Xgate\Zgate$.
}
\label{fig:R}
\end{figure}
%
As was shown in Section 4 of~\cite{Low:2016znh}, it is given by
\begin{align}
\label{eq:Whdefqas}
\begin{aligned}
W_H =&  (\Hgate_q\otimes\unit_{as})
(R_{qa}\otimes\unit_s)
(\Xgate_q\otimes\unit_{as})
\\
&
\times
% (\unit_a\otimes
U'_{qas}
(\Hgate_q\otimes\unit_{as}) \,,
\end{aligned}
\end{align}
%
where $\Hgate_q$ and $\Xgate_a$ are the Hadamard and X gate on the qubit $\sket{q}$, $R_{qa}$ is a standard reflection operator
\begin{align}
    \label{eq:refl}
    R_{qa} = 2 \sket{g}_a \sket{+}_q \sbra{+}_q \sbra{g}_a - \unit_{qa}
    \,,
\end{align}
%
and
\begin{align}
    U'_{qas} = \sket{0}_q \sbra{0}_q U_H + \sket{1}_q \sbra{1}_q U_H^\dagger
    \,,
\end{align}
%
is an operator that applies the $U_H$ or $U_H^\dagger$ operator, depending on the state of $\sket{q}$. 

One can show through explicit computation that
%
\begin{align}
    W_H \sket{g}_{qa} \sket{\lambda}_s &= \left( \lambda\, \sket{g}_{qa} - \sqrt{1-\lambda^2} \sket{\bot^\lambda}_{qa} \right)\sket{\lambda}_s
    \,,
\end{align}
%
with
%
\begin{align}
    \sket{\bot^\lambda}_{qa} = \sket{-}_q \sket{\bot^\lambda}_a
    \,,
\end{align}
verifying that \cref{eq:Whdef} gives indeed a qubitized BE of $H$. 

The circuits for operators $W_H$, $U'_{qas}$, and $R_{qa}$ are shown in~\cref{fig:BEW,fig:R}.
\MK{Note that while the circuit for $W_H$ shown in \Cref{fig:BEW} if fully general and can be used for arbitrary $U_H$, more efficient constructions are available for block encodings considered in this work.
In particular, when $U_H$ is assembled from \PREPARE and \SELECT operators as in~\cref{eq:lcube}, and if additionally $\SELECT^2=\unit$ (which holds for the \SELECT operator defined in~\cref{eq:lcuselect}), then $W_H$ can be constructed as~\cite{Low:2016znh,Babbush:2018ywg}
}
\begin{equation}
    \label{eq:WRS}
    W_H = R_\beta \cdot \SELECT \,,
\end{equation}
\MK{where $R_\beta$ is the reflection with respect to $\sket{\beta_a}$ defined in~\cref{eq:prepstate}:}
\begin{equation}
    R_\beta = 2 \sket{\beta}_a\sbra{\beta}_a\otimes\unit_s - \unit_{as} \,.
\end{equation}
\MK{The controlled version of $W_H$ operator (which we use in the construction of $V_H^{(\theta)}(\phi)$ in \Cref{sec:qsptimeevol} below) can then be implemented as shown in Fig.~1 in Ref.~\cite{Babbush:2018ywg}.}

This qubitized BE $W_H$ gives the same result as the original BE $U_H$ when acted on $\sket{g}_{qa} \sket{\lambda}_s$, but it has a much simpler structure when applied multiple times. 
%
Since $W_H$ is block diagonal, one finds\footnote{Note that ~\cref{eq:wwtilde,eq:wwtildematrix} ...}
%
\begin{align}
\label{eq:oneWone}
    \left(\unit_{qa} \otimes \sbra{\lambda'}_s \right) \left(W_H\right)^k \left(\unit_{qa} \otimes \sket{\lambda}_s \right) = \left(\widetilde{W}_H^{(\lambda)}\right)^k\delta_{\lambda' \lambda}
    \,,
\end{align}
%
and one can show that \CFK{as we already calculated the matrix elements in this subspace explicitly in Eq 41, we could skip it in this step to save space?}
%
% \begin{align}
% \label{eq:WHkmatr}
% \begin{aligned}
%     \left(W_H^{(\lambda)}\right)^k &= \begin{pmatrix} T_k(\lambda) & - \sqrt{1-\lambda^2} \, U_{k-1}(\lambda)\\ \sqrt{1-\lambda^2} \, U_{k-1}(\lambda) & T_k(\lambda) \end{pmatrix}_{qa}\\
%     &= \exp \left( -i (Y_{qa} \otimes \unit_{s}) k \theta_\lambda \right)
%     .
% \end{aligned}
% \end{align}
% \MK{Here is the corrected version of the previous equation, assuming that the definition from \cref{eq:oneWone} holds and $W_H^{(\lambda)}$ carries the $qa$ indices:}
% \begin{align}
% \label{eq:WHkmatr}
% \begin{aligned}
% \left(W_H^{(\lambda)}\right)^k&= \begin{pmatrix} T_k(\lambda) & - \sqrt{1-\lambda^2} \, U_{k-1}(\lambda)  \\ \sqrt{1-\lambda^2} \, U_{k-1}(\lambda) & T_k(\lambda) \end{pmatrix}_{qa}
% \\
%     &= \exp \left( -i Y_{qa} k \theta_\lambda \right)
%     .
% \end{aligned}
% \end{align}
\begin{align}
\label{eq:wwtildematrixpowerk}
\begin{aligned}
\left(W_H^{(\lambda)}\right)^k &= \begin{pmatrix} \sbra{g}_a \left(\widetilde{W}_H^{(\lambda)}\right)^k \sket{g}_a & \sbra{g}_a \left(\widetilde{W}_H^{(\lambda)}\right)^k \sket{\bot^\lambda}_a \\  \sbra{\bot^\lambda}_a  \left(\widetilde{W}_H^{(\lambda)}\right)^k \sket{g}_a & \sbra{\bot^\lambda}_a  \left(\widetilde{W}_H^{(\lambda)}\right)^k \sket{\bot^\lambda}_a \end{pmatrix}_{h_{qa}^{(\lambda)}}
    \\
    &=\begin{pmatrix} T_k(\lambda) & - \sqrt{1-\lambda^2} \, U_{k-1}(\lambda)  \\ \sqrt{1-\lambda^2} \, U_{k-1}(\lambda) & T_k(\lambda) \end{pmatrix}_{h_{qa}^{(\lambda)}}
    \\&=
    \exp \left( -i Y k \theta_\lambda \right).
\end{aligned}
\end{align}

Here $T_k(\lambda)$ and $U_k(\lambda)$ are Chebyshev polynomials of the first and second kind, respectively. 
%
Given that Chebyshev polynomials are an excellent 
polynomial basis for approximating $L^\infty$ functions on an finite interval, one can hope to construct a general function of the eigenvalues (and therefore of the Hamiltonian matrix itself) by combining powers of the $W_H$ operator. 
%
In the next section we discuss how the time evolution operator can be approximated using this technique. 

\subsubsection{Calculating the time evolution operator using QSP\label{sec:qsptimeevol}}
\begin{figure*}[t]
\begin{quantikz}
\lstick{$\sket{0}_b$} & \gate{\Hgate} & \gate[4]{V_H^{(\theta)}(\phi_{1})} & \gate[4]{V_H^{(\theta)}(\phi_{2})} & \qw \ \cdots \ & \gate[4]{V_H^{(\theta)}(\phi_{\Nphi})} & \gate{\Hgate} & \meter{} & \setwiretype{c} \rstick{0} \\
\lstick{$\sket{0}_q$} & \gate{\Hgate} &  & & \qw \ \cdots \ & & \gate{\Hgate} & \meter{} & \setwiretype{c} \rstick{0}  \\
\lstick{$\sket{0}_a$} & \qw \qwbundle{} & & \qw \cdots & \qw \ \cdots \ & & \qw & \meter{} & \setwiretype{c} \rstick{0}  \\
\lstick{$\sket{\psi}_s$} & \qw \qwbundle{} & & & \qw \ \cdots \ & & \qw & \qw & \qw \rstick{$\approx \me^{-iHt}\sket{\psi}$}
\end{quantikz}
\caption{Quantum Signal Processing (QSP) circuit used for simulating time evolution, reproduced from Ref.~\cite{Novikau:2021yra}.
The circuit prepares a block encoding for the approximation of the time evolution operator $\me^{-iHt}\sket{\psi}$.
Circuit for $V_H^{(\theta)}(\phi)$ is shown in~\cref{fig:VH}.
When all the ancillary qubits are measured in the zero states, the desired operator is applied to the system register $\sket{\psi}_s$.
Without loss of generality, $\sket{g}_a$ is set to $\sket{g}_a=\sket{0}_a$.
}
\label{fig:QSP}
\end{figure*}
\begin{figure}[t]
\begin{quantikz}
\lstick{$\sket{}_b$} & \gate{R_z(-\frac{\phi}{2})} & \gate{\Hgate} & \ctrl{1} & \gate{\Hgate} & \gate{R_z(\frac{\phi}{2})} & \\
\lstick{$\sket{}_q$} & \phantomgate{R_z(-\frac{\phi}{2})} & & \gate[3]{W_H} & & & \\
\lstick{$\sket{}_a$} & \phantomgate{R_z(-\frac{\phi}{2})} \qwbundle{} & & & & & \\
\lstick{$\sket{}_s$} & \phantomgate{R_z(-\frac{\phi}{2})}\qwbundle{} & & & & &
\end{quantikz}
\caption{Circuit for $V_H^{(\theta)}(\phi)$, as defined is~\cref{eq:VHphi}.}
\label{fig:VH}
\end{figure}
% \begin{figure*}[t]
% \begin{quantikz}
% \lstick{$\sket{}_b$} & \gate[4]{V^{(\theta)}_H(\phi)} & \phantomgate{\frac{\phi}{2}} \\
% \lstick{$\sket{}_q$} & & \phantomgate{\frac{\phi}{2}} \\
% \lstick{$\sket{}_a$} & \qwbundle{} & \phantomgate{\frac{\phi}{2}} \\
% \lstick{$\sket{}_s$} & \qwbundle{} &  \phantomgate{\frac{\phi}{2}}
% \end{quantikz}=
% \begin{quantikz}
% \lstick{$\sket{}_b$} & \gate{R_z(-\frac{\phi}{2})} & \gate{\Hgate} & \ctrl{1} & \gate{\Hgate} & \gate{R_z(\frac{\phi}{2})} & \\
% \lstick{$\sket{}_q$} & \phantomgate{R_z(-\frac{\phi}{2})} & & \gate[3]{W_H} & & & \\
% \lstick{$\sket{}_a$} & \phantomgate{R_z(-\frac{\phi}{2})} \qwbundle{} & & & & & \\
% \lstick{$\sket{}_s$} & \phantomgate{R_z(-\frac{\phi}{2})}\qwbundle{} & & & & &
% \end{quantikz}
% \caption{Circuit for $V_H^{(\theta)}(\phi)$, as defined is~\cref{eq:VHphi}.}
% \label{fig:VH}
% \end{figure*}
In order to use the operator $W_H$ of the previous section to calculate the exponential of the Hamiltonian, we first note that the qubitized operator $W_H$ can be diagonalized by defining the states
%
\begin{align}
    \sket{\theta_\pm^\lambda}_{qas} \equiv \frac{1}{\sqrt{2}} \left( \sket{g}_{qa} \pm i \sket{\bot^\lambda}_{qa} \right)\sket{\lambda}_s
    \,.
\end{align}
%
Using \cref{eq:Whdef} one can easily show that
%
\begin{align}
    W_H \sket{\theta_\pm^\lambda}_{qas} = \me^{i \theta_\pm^\lambda}\sket{\theta_\pm^\lambda}_{qas}
    \,,
\end{align}
%
with
%
\begin{align}
    \theta_\pm^\lambda = \mp \arccos(\lambda)
    \,.
\end{align}

Given this form, one can now define a new operator $V_H(\phi)$, which depends on the value of an angle $\phi$ and which can be constructed from the operator $W_H$. 
%
It requires one more ancillary qubit $\sket{b} \in {\cal H}_b$, such that the operator $V_H(\phi)$ acts on the Hilbert space ${\cal H}_{bqas}  \equiv {\cal H}_b \otimes {\cal H}_q \otimes {\cal H}_a \otimes {\cal H}_s$. 
%
It is defined by (see~\cref{fig:VH})
%
\begin{align}
    V_H(\phi) = (\me^{-i \phi Z_b/2}\otimes \unit_{qas}) W' (\me^{i \phi Z_b/2}\otimes \unit_{qas})
    \,,
\end{align}
%
where $Z_b$ is the usual Pauli $Z$ operator acting on the qubit $\sket{b}$, and $\tilde W$ is the $W_H$ operator controlled on the $\sket{b}$, which now acts on the Hilbert space ${\cal H}_{bqas}$:
%
\begin{align}
    W' = \unit_{qas} \sket{+}_b \sbra{+}_b + W_H \sket{-}_b \sbra{-}_b
    \,.
\end{align}

One can show through explicit computation that
%
\begin{align}
    & \left(\unit_b \otimes \sbra{\theta^{\lambda'}_\pm}_{qas}\right)
    V_H(\phi)\left(\unit_b \otimes \sket{\theta^{\lambda}_\pm}_{qas}\right) \nonumber\\
    & \qquad \qquad = V_H^{(\theta^\lambda_\pm)} (\phi) \, \delta_{\lambda \lambda'}
    \,,
\end{align}
%
with
%
\begin{align}
\label{eq:VHphi}
\begin{aligned}
    V_H^{(\theta)}(\phi) &=     
    \me^{i \frac{\theta}{2}}\begin{pmatrix}
    \cos\frac{\theta}{2} & - i \sin\frac{\theta}{2}\me^{-i \phi} \\
    - i \sin\frac{\theta}{2}\me^{i \phi} & \cos\frac{\theta}{2}
    \end{pmatrix}_b \\
    &= \me^{i \frac{\theta}{2}} \me^{-i \frac{\theta}{2}\left(X_b \cos\phi + Y_b \sin\phi \right)}
    \,,
\end{aligned}
\end{align}
%
where $X_b$ and $Y_b$ denote the Pauli-$x$ and $y$ matrices in ${\cal H}_b$. 

What this construction has accomplished is to create a unitary operator $V_H(\phi)$ that is block diagonal in the original Hilbert space ${\cal H}_s$, with the entries of the $2 \times 2$ matrix in ${\cal H}_b$ given by functions of the eigenvalues of the Hamiltonian (through $\cos \theta_\pm^\lambda$), parameterized by some $\phi$. 
%
By multiplying several of these operators in sequence (each with a different value of~$\phi$),
%
\begin{align}
    V_H^{(\theta)}(\vec \phi) \equiv V_H^{(\theta)}(\phi_{\Nphi}) \ldots V_H^{(\theta)}(\phi_{1})\,,
\end{align}
one obtains an operator that is still block diagonal in ${\cal H}_s$. 
%
$V_H^{(\theta)}(\vec \phi)$ is a $2\times 2$ matrix in ${\cal H}_b$, which can be expressed using the Pauli decomposition
%
\begin{align}
\label{eq:VHGeneralMatrix}
    V_H^{(\theta)}(\vec \phi) = A(\theta) \unit_b + i B(\theta) X_b + i C(\theta)Y_b + i D(\theta) Z_b
    \,.
\end{align}
%
The functions $A(\theta) \ldots D(\theta)$ are all parameterized by the angles $\vec\phi = (\phi_1, \ldots, \phi_{\Nphi})$. 
%
The type of functions that can be obtained for different choices of $\vec(\phi)$ were studied in~\cite{Low:2016jxt} and it was shown that one can choose values of $\vec\phi$ to obtain functions $A$ and $C$ of the form
\begin{align}
\begin{aligned}
    |A^2(\theta)|&  + |C^2(\theta)| \leq 1 \,, \qquad
    A(0) = 1\\
    A(\theta) &= \sum_{k=0}^{{\Nphi}/2} a_k \cos (k\theta)\\
    C(\theta) &= \sum_{k=1}^{\Nphi/2} c_k \sin (k\theta)
\,.
\end{aligned}
\end{align}
%
Reversing this logic, one can start from some desired functions $A(\theta)$, $C(\theta)$, and determine phases $\vec{\phi}$ such that $V_H^{(\theta)}(\vec \phi)$ reproduces these functions (approximately). 
%
This can be accomplished using an efficient classical procedure given in Ref.~\cite{Low:2016jxt}.\footnote{A recent version of QSP, \emph{generalized QSP}, significantly improves the cost of calculating phases~$\vec{\phi}$~\cite{Motlagh:2023oqc}.}

We omit now a few final details, all of which are straightforward and can  be found in Ref.~\cite{Low:2016znh}, and simply state the relevant results. 
%
As can be confirmed from~\cref{eq:VHGeneralMatrix}, letting the operator $V_H^{(\theta)}(\vec \phi)$ act on the state $\sket{+}_b$ and post-selecting on $\sbra{+}_b$ picks out the function 
%
\begin{equation}
\label{eq:Vfinal}
\begin{aligned}    \sbra{+}_b\sbra{g}_{qa} \sbra{\lambda'}_s &V_H(\vec \phi)\sket{+}_b\sket{g}_{qa} \sket{\lambda}_s\\
    & \qquad = \delta_{\lambda \lambda'} \left[ \tilde A(\lambda) + i \tilde C(\lambda) \right]
    .
\end{aligned}    
\end{equation}    
%
The functions $\tilde A(\lambda)$ and $\tilde C(\lambda)$ are directly related to the functions $A(\theta_\lambda)$, $C(\theta_\lambda)$, with the detailed relation given in Ref.~\cite{Low:2016znh}. 
%
The success probability for measuring the system in the state $\sket{+}_b\sket{g}_{qa}$ for a given value $\lambda$ depends on the functions and is given by 
\begin{align}
\label{eq:QSP_p_def}
    p \geq |\tilde A^2(\lambda)| + |\tilde C^2(\lambda)|
    \,.
\end{align}
%
An efficient classical algorithm exists that finds phases $\vec\phi$ such that one can approximate the time evolution operator with uncertainty bounded by $\varepsilon$
%
\begin{align}
\label{eq:qspapprox}
    \left| \me^{i \lambda \tilde{t}} - [\tilde A(\lambda) + i \tilde C(\lambda)] \right| < \varepsilon
    \,.
\end{align}
%
This is related to the fact that products of qubitized BEs give rise to Chebyshev polynomials, which can be used to approximate the real and imaginary part of $\me^{i \lambda t}$ through the Jacobi-Anger expansion.
%
In this case, the circuit in \cref{fig:QSP} would implement the approximate BE of the evolution operator $\me^{-iHt}$.
%
The number of phases needed for a given value of $\varepsilon$ is bounded by 
\begin{align}
    \label{eq:nphi}
    \Nphi = \OO\!\left(\tilde{t} + \log(1/\varepsilon)\right) = \OO\!\left(\alpha t + \log(1/\varepsilon)\right)
    .
\end{align}
%
Note also that~\cref{eq:QSP_p_def,eq:qspapprox} imply that 
%
\begin{align}
    p \geq 1 - \OO(\varepsilon)
    \,,
\end{align}
since the time evolution operator has unit magnitude.

It is worth mentioning that the success rate of QSP is always $\OO(1)$, independent of the success rate of the BE used. 
%
This is due to the fact that we have used QSP to implement a unitary function ($\me^{-i H t}$) which has unit norm. 
%
This implies that $\tilde A(\lambda)^2 + \tilde C(\lambda)^2 \approx 1$, which together with \cref{eq:QSP_p_def} gives a success probability that is close to one.


Before we conclude, we should mention that we have focused here on using QSP to simulate the time evolution operator, which required a particular form of the polynomial functions. 
%
QSP is more general than that, and other functions can be implemented as well, some of which require less resources than the case discussed here.
%
For more details, we find ~\cite{Lin:2022vrd} a useful reference.

\subsection{HHKL}
\label{sec:hhkl}
The results presented so far (PFs and QSP) can be applied to general site-local Hamiltonians (see~\cref{def:loclattice}).
%
For geometrically-site-local Hamiltonians (see~\cref{def:geomloclattice}) one can use the fact that information from one area of the lattice can only spread to areas not directly connected to it through repeated actions of the time evolution operators, which implies that the speed with which this information spreads is bounded. 
%
This is formalized by the Lieb-Robinson bound~\cite{Lieb:1972wy}.
%
This idea was used in a paper by Haah, Hastings, Kothari and Low (HHKL)~\cite{Haah:2018ekc} to devise a scheme for simulating the time evolution of geometrically-site-local Hamiltonians. 

As before, this section is aimed at giving the reader a basic understanding of the technique, without going into too many of the details. 
%
In order to understand these details the reader is encouraged to read the excellent description of the algorithm in the original work, where all statements are also carefully proved. 

The main ingredient to the HHKL algorithm is that the time evolution of a large quantum system with geometrically local Hamiltonian can be obtained from the time evolution of two smaller systems that share some overlap, which has to be of at least the size given by the ball of size $\OO(1)$ used in~\cref{def:geomloclattice}. 
% \NM{I think we need to change this now that Definition 3 no longer introduces the parameter $\gloc$.}
%
Thus, the system Hilbert space ${\cal H}_s$ is divided into three parts, ${\cal H}_{a,b,c}$ such that ${\cal H}_s = {\cal H}_a \otimes {\cal H}_b \otimes {\cal H}_c$.
%
In the discussion of Ref. ~\cite{Haah:2018ekc} is assumed that the local Hamiltonian $H_J$ such that $||H_J|| \leq 1$. Thus, in the remainder we work with 
\begin{align}
    \tilde{H}_J = \frac{H_J}{||H_J||}\,, \qquad \tilde{t} = ||H_J|| t
    \,.
\end{align}
%
First, one uses that the evolution of a system for some long time $\tilde{t}$ can be split into the product of unitaries over shorter times $\Delta t=\OO(1)$:
%
\begin{align}
    U(\tilde{t}, 0) = U(\tilde{t}, \tilde{t}-\Delta t) \cdots U(\Delta t,0)
    \,.
\end{align}
The total number of such unitaries is $\OO(\tilde{t})$.

Lemma 6 of Ref.~\cite{Haah:2018ekc} states that the time evolution $U_s(\Delta t)$ of a Hamiltonian on the whole system over time $\Delta t$ can be obtained by multiplying together the forward time evolution in the system ${\cal H}_{b\cup  c} = {\cal H}_b \otimes {\cal H}_c$ and ${\cal H}_{b\cup c} = {\cal H}_b \otimes {\cal H}_c$ and the backwards evolution in the system ${\cal H}_b$ as
%
\begin{align}
    \label{eq:hhklmain}
    U_{a\cup b\cup c}(\Delta t) = U_{a\cup b}(\Delta t) U^\dagger_b(\Delta t) U_{b\cup c}(\Delta t)  + \OO(\delta)
    \,,
\end{align}
where the error in the approximation is given by
%=
\begin{align}
\label{eq:HHKL_delta_def}
    \delta \equiv \delta(a,b,c) &= \me^{-\mu \, {\rm d}(a,c)} \sum_{X\in {\rm BD}(ab,c)}||\tilde{H}_X||
    \,.
\end{align}
%
For now we assume that each of the $U(\Delta t)$ on the RHS of~\cref{eq:hhklmain} is implemented exactly. 
%
In~\cref{eq:HHKL_delta_def} $\mu$ is some constant, ${\rm d}(a,c)$ is the smallest distance between any point in $a$ and $c$, and the norm $||\tilde{H}_J||$ is summed over all terms that are on the boundary of $a\cup b$ and $c$, indicated by ${\rm BD}(ab,c)$. The total number of terms in this sum is $\OO(\ell^{\dims-1})$. 
%
The uncertainty is therefore exponentially suppressed in the distance between the regions $a$ and $c$.
%
This implies that this approximation works well for large enough distance $\ell \equiv {\rm d}(a,c)$.

This result can be applied recursively, splitting the evolution into smaller and smaller pieces, which just have to be larger than the size of the ball $\OO(1)$.
%
If the size of the original system is given by $L^\dims$ and the final pieces contain order $\ell^\dims$ lattice sites, one ends up with 
\begin{align}
    m = \OO\left(\frac{L^\dims}{\ell^\dims}\right)
\end{align}
individual pieces. 
%
Taking into account the $\tilde  t$ evolution operators we started from, the final error in the evolution is given by $\tilde t\, m , \delta$. 
%
In order to have the final error of order the exponentiation error $\varepsilon$ therefore requires 
%
\begin{align}
\label{eq:delta_def}
    \delta = \OO\left( \frac{\varepsilon}{\tilde{t} \, m} \right)
    .
\end{align}
%
Equating \cref{eq:HHKL_delta_def,eq:delta_def} one finds that this can be satisfied if one uses
%
\begin{align}
    \ell = \Theta\left( \log \left( \frac{L^\dims \tilde{t}}{\varepsilon} \right)\right)
    .
\end{align}

One can then estimate the required resources using the fact that one needs to compute 
%
\begin{align}
    \OO(T m) = \OO\left( L^\dims \tilde{t} \log^{-\dims}\left(\frac{L^\dims \tilde{t}}{\eps} \right)\right)
\end{align}
time evolution operators on a system of size $\OO(\ell^\dims)$.\footnote{Note that decreasing $\eps$ is logarithmically decreasing the number of evolution operators. This number clearly has to be larger than unity, meaning $\eps$ cannot be exponentially small with system size.}
%
The cost and the associated additional error for implementing each of these ``local'' pieces depends on the algorithm used for their implementation. 


\subsection{QETU}
\begin{figure*}[t]
    % \large
    \centering
    \begin{quantikz}[row sep={1cm,between origins}, column sep=0.25cm]
        \lstick{$\sket{0}$} & \qw & \gate{\me^{i \tilde{\varphi}_{0} X}} & \ctrl{1} & \gate{\me^{i \tilde{\varphi}_{1} X}} & \ctrl{1} & \qw & \ldots\ & \qw &  \ctrl{1} & \gate{\me^{i \tilde{\varphi}_{1} X}} & \ctrl{1} & \gate{\me^{i \tilde{\varphi}_{0} X}} &\qw & \meter{} & \setwiretype{c} \rstick{0} 
        \\
        \lstick{$\sket{\psi}$} & \qw & \qw & \gate{U} & \qw & \gate{U^\dagger} & \qw & \ldots\ & \qw & \gate{U} & \qw & \gate{U^\dagger} & \qw & \qw & \qw & \rstick{$\frac{F(\cos(A/2)) \sket{\psi}}{||F(\cos(A/2)) \sket{\psi}||}$}
    \end{quantikz}
    \caption{Circuit diagram for QETU. The top qubit is the control qubit and the bottom register is the state that the matrix function is applied to.
    Here $U = \me^{-i \tau A}$ is the time evolution circuit.
    If the control qubit is measured to in the zero state, one prepares the normalized quantum state $F(\cos(\tau A/2))\sket{\psi}/||F(\cos(\tau A/2)) \sket{\psi}||$ for some even polynomial $F(x)$.
    For symmetric phase factors $(\tilde{\varphi}_0, \tilde{\varphi}_1, \dots, \tilde{\varphi}_1, \tilde{\varphi}_0) \in \mathds{R}^{d+1}$, the function $F(x)$ is a real even polynomial of degree $d$. 
    The probability of measuring the control qubit in the zero state is $p = ||F(\cos(\tau A/2)) \sket{\psi}||^2$.}
    \label{fig:qetu_circ}
\end{figure*}

In this section, we review the Quantum Eigenvalue Transformation for Unitary Matrices (QETU) developed in Ref.~\cite{Dong:2022mmq}.
%
We then describe a novel application of QETU to implement BEs based off a method in Ref.~\cite{Kane:2023jdo}. 
%
In this section we only discuss the details relevant to our implementation, and further details can be found in the original references.

The Quantum Eigenvalue Transformation for Unitary Matrices (QETU) is very similar to the QSP method described in Sec.~\ref{sec:QSP} in that it allows one to implement general matrix functions of some Hermitian operator $A$ by performing repeated calls to some fundamental building block. 
%
The major difference of QETU is that, instead of performing repeated calls to a BE $U_A$ as with QSP, the building block for QETU is the time-evolution operator $\me^{-i \tau A}$ for some small time $\tau$.
%
The ``U'' in QETU indicates that the building block in the circuit is a unitary matrix.
%
In a broad sense, QETU replaces the BE $U_A$ in the QSP circuit in \cref{fig:QSP} with the controlled time-evolution operator $\me^{-i \tau A}$. 
%
One major difference is that QETU implements real functions with definite parity.
%
Constructing functions without definite parity or complex functions can be achieved by using QETU to implement the components with definite parity, and then using LCU to add the pieces together.

The QETU circuit is shown in \cref{fig:qetu_circ}. 
%
One nice property of QETU is that it requires only a single ancillary qubit, the so-called control qubit.
%
By repeatedly performing controlled calls to $U = \me^{-i \tau A}$ alternated with rotation gates and post-selecting the control qubit on the zero state, one implements the even matrix function $F(\cos(\tau A/2))$ on the state register\footnote{QETU relies on repeated calls to the controlled implementations of the time-evolution operator. While this does not change the asymptotic scaling, it introduces a large prefactor in the gate complexity. A control-free version of QETU was also presented in Ref.~\cite{Dong:2022mmq}, which involves an operator dependent procedure. The procedure for diagonal Hermitian matrices can be found in Appendix B of Ref.~\cite{Kane:2023jdo}.}, where the function $F$ is parameterized by the angles $\vec(\phi)$, similar to the case in QSP.
%
As was done there, we require $|F(x)| \leq 1 \forall x \in [-1, 1]$.
The success probability of measuring the control qubit in the zero state is $||F(\cos(\tau A/2))\sket{\psi}||$\footnote{Note that the original algorithm set $\tau = 1$. It was shown in Ref.~\cite{Kane:2023jdo}, however, that allowing $\tau$ to be a free parameter can reduce the cost of QETU for both ground-state preparation and implementation of Gaussian wavepackets.}.     
In practice, the QETU circuit is used for approximately implementing $\fex(A)$ by realizing a transformation $F(\cos (\tau A/2))$, where $F(x)$ is a polynomial approximation to $\Fex(x)\equiv \fex(\frac{2}{\tau}\arccos(x))$.
We now describe our proposal for implementing BEs using QETU.

Suppose we want to prepare some function $\fex(A)$ of a diagonal Hermitian matrix $A$ with known eigenvalues $A \sket{a_j} = a_j \sket{a_j}$.
Furthermore, define $a_\text{max} \equiv \max(a_j)$ and $a_\text{min} \equiv \min(a_j)$.
Because QETU returns a function of a periodic argument, \textit{i.e.} $F(\cos(\tau A/2))$, any function constructed using QETU will repeat itself for large values of $a_j$. 
To avoid this complication, the original algorithm \cite{Dong:2022mmq} proposed to shift the spectrum of $A$ to the limited range $[\eta, \pi-\eta]$ for some $\eta>0$. 
This was crucial to guarantee isolation of the ground state when using QETU for state preparation. 
Furthermore, it was shown in Ref.~\cite{Kane:2023jdo} that shifting the spectrum of the operator $A$ to be in this limited range and allowing $\eta$ to be a free parameter dramatically improved the convergence of the Chebyshev approximation to functions of the form $\fex(A) \sim \me^{-A^2 / \sigma^2}$.
The shifted operator $A_\text{sh}$ whose spectrum is in the range $[\eta, \pi-\eta]$ is given by
%
\begin{equation}
    A_\text{sh} = c_1 A + c_2\,,
\end{equation}
%
where
%
\begin{equation}
    c_1 = \frac{\pi - 2\eta}{a_\text{max} - a_\text{min}}\,, \quad c_2 = \eta - c_1 a_\text{min}\,.
\end{equation}


Note that using $\me^{-i \tau A_\text{sh}}$ as the building block in the QETU algorithm requires a modification to the function $\Fex(x)$.
The desired function must satisfy $\Fex(\cos(\tau A_\text{sh}/2) = \fex(A)$, which implies
%
\begin{equation}
    \Fex(x) = \fex\!\left(\frac{\frac{2}{\tau}\arccos(x) - c_2}{c_1}\right).
\end{equation}
%
Now that we know the form of the function we wish to approximate, we make several observations.

First, even if the function $\fex(x)$ has definite parity, the function $\Fex(x)$ will in general not have definite parity due to the presence of the $\arccos(x)$. 
This implies that one will have to implement the even and odd pieces of $\Fex(x)$ separately, and then add them using LCU. 
While there are no theoretical issues with this procedure for this application, it was found in Ref.~\cite{Kane:2023jdo} that using LCU introduced a large prefactor, and that the need to use LCU could be avoided altogether by choosing $\tau$ in such a way as to make $\Fex(x)$ have definite parity.
To see this, note that if one chooses $\tau = \pi/c_2$, the function $\Fex(x)$ becomes
%
\begin{equation}
    \Fex(x) = \fex\!\left(-\frac{2}{\pi} \frac{c_2}{c_1} \arcsin(x) \right),
\end{equation}
%
where we have used $\arcsin(x) = \pi/2 - \arccos(x)$.
Because $\arcsin(x)$ has odd parity, the function $\Fex(x)$ has the same parity as the function $\fex(x)$, as desired.
Note that $\tau$ is a function of $\eta$ through the parameter $c_2$, and one must choose a different $\tau$ for each $\eta$.

The second observation we make regarding $\Fex(x)$ is that, for general functions $\fex(x)$, its first derivative diverges at $x = \pm 1$ due to the presence of the $\arcsin(x)$ (or $\arccos(x)$) term.
Chebyshev approximations of functions with $m$ continuous derivatives on $x \in [-1,1]$ are known to converge polynomially to the true function with the typical rate $(1/n_\text{Ch})^m$, where $n_\text{Ch}$ is the number of Chebyshev polynomials used in the approximation~\cite{trefethen_apprx_theory}.
If one needed to reproduce $\Fex(x)$ for all $x \in [-1,1]$, this poor convergence would spoil the optimal scaling with precision.
We now outline a method for overcoming this problem described in Ref.~\cite{Kane:2023jdo}.

The key method we employ from Ref.~\cite{Kane:2023jdo} is to exploit the fact that the spectrum of the operator $A_\text{sh}$ is known exactly (in our case, operators given in \cref{eq:phidig,eq:pidig} below play the role of $A_\text{sh}$), and therefore one only samples $\Fex(x)$ at those finitely many points. 
%
Because there are $\OO(2^{\nq})$ such values, one can reproduce the function at those points exactly by using $\OO(2^{\nq})$ Chebyshev polynomials.
%
In this way, one avoids the poor polynomial convergence of the Chebyshev expansion at the cost of introducing an exponential scaling with $\nq$.
%
However, because digitization errors generally decrease exponentially with $\nq$, one needs only small values of $\nq$ and this exponential scaling will not be a computational bottleneck\footnote{Note that it was found in Ref.~\cite{Kane:2023jdo} that by increasing $\eta$, this polynomial convergence with the degree of the Chebyshev polynomial can be converted to exponential for the class of functions of the form $\fex(x) = \me^{-x^2/\sigma^2}$.
%
One issue with applying this method to our problem of $\fex(x) = x^n$ is that, as $\eta$ increases, the scale factor $\alpha$ diverges as $\eta \to \pi/2$, as can be seen in Eq.~\eqref{eq:c2overc1}. 
%
For this reason, we fix $\eta=0$ and produce the function exactly, and leave further optimizations for future work.}.

Once the Chebyshev polynomial has been determined, the next step is to calculate the phases $\varphi$ appearing in the circuit in Fig.~\ref{fig:qetu_circ}
%
The procedure to do this is given in Ref.~\cite{Dong:2022mmq}, and an example code to calculate the phases has been implemented in QSPPACK~\cite{qsppack}.
%
Note that the classical cost of determining the phases was found to scale roughly quadratically with the number of phases.~\cite{Kane:2023jdo}.
%
As described in Appendix B of Ref.~\cite{Dong:2022mmq}, the phases in the QETU circuit $\{\tilde{\varphi}_j \}$ are related to the phases calculated using QSPPACK $\{\tilde{\phi}_j\}$ by $\tilde{\varphi}_j = \tilde{\phi}_j + (2-\delta_{j\, 0}) \pi/4$.
\CFK{state construction of $S$ operator}


\subsection{Summary and precise statement of techniques used}
\label{sec:methods_summary}

\subsubsection{General product formulas}
\begin{definition}
    A $p^{\text{th}}$ order PF $S_p(t)$ is a PF of the form~\eqref{def:PF}, such that it approximates the true exponential $\me^{-iHt}$ to $p^{\text{th}}$ order in $t$, i.e.,
    \begin{equation}
        \label{eq:pth_order_PF}
        \me^{-iHt} = S_p(t) + \mathcal{O}(t^{p+1})\,.
    \end{equation}
\end{definition}

\begin{theorem}
[Trotter number with commutator scaling]
\label{them:childs_pf}
        Let $H = \sum_{\gamma=1}^{\Gamma}H_\gamma$ be an operator comprised of $\Gamma$ Hermitian summands. Let $S_p(t)$ be a $p^{\text{th}}$ order PF as defined by \eqref{eq:pth_order_PF}, with $t \geq 0$. Then, if we require an exponentiation error $\mathcal{O}(\varepsilon)$, as defined by \eqref{eq:exp_error}, it suffices to choose
        \begin{equation}\label{eq:trotter_number}
            r = \OO\!\left( \frac{\Tilde{\alpha}^{\frac{1}{p}}t^{1 + \frac{1}{p}}}{\varepsilon^{\frac{1}{p}}} \right)
            ,
        \end{equation}
        where $\Tilde{\alpha} \equiv \sum_{\gamma_1,\gamma_2,...,\gamma_{p+1} = 1}^{\Gamma} \lvert\lvert [ H_{\gamma_{p+1}},... [H_{\gamma_2},H_{\gamma_1}] ] \rvert\rvert$
\end{theorem}
\begin{proof}
    This theorem follows directly from Theorem 11 and Corollary 12 of~\cite{Childs:2019hts}.
\end{proof}



\subsubsection{Quantum Signal Processing}
\label{sec:QSP}
In this section we summarize the results of the section on QSP in a concise and precise form which will be referred to later in the text.

\begin{definition}
[Block encoding]
\label{def:be}
Let $H$ be a Hamiltonian acting on the $n$-qubit Hilbert space $\mathcal H_s\cong \mathbb C^{2^n}$.
%
Let $k \ge  0$ be an integer and let $U_H$ be a unitary operator on the joint Hilbert space $\mathcal H_a \otimes \mathcal H_s$, where $\mathcal H_a \cong \mathbb C^{2^k}$ denotes the Hilbert space of $k$ ancillas.
%
Then, for $\alpha\in \mathbb R^+$, the unitary operator $U_A$ is called an $(\alpha,k)$\textit{-block-encoding} of $A$ if for every state $\sket{\psi} \in \mathcal H_s$:
%
\begin{equation}
\label{eq:lcusimple}
\left(\unit_{s}\otimes \sbra{g}_g\right)U_A \left(\unit_s\otimes \sket{g}_a\right) = A/\alpha\,,
\end{equation}
%
where $\sket{g}_a$ is some state in $\mathcal H_a$, $\unit_{s}$ is the identity operator on $\mathcal H_s$.
%
The value $\alpha$ chosen such that $\|A\|/\alpha \leq 1$ is called the \textit{scale factor} of the BE.
\end{definition}

BEs can be constructed using LCU as follows
\begin{lemma}
[LCU block encoding]
\label{LCU}
    Let $U_0, \ldots, U_{M-1}$ be $M$ unitary operators acting on a system Hilbert space ${\cal H}_s$ and define the operator $T = \sum_{i=0}^{M-1} \beta_i U_i$. The LCU method provides a $(\beta, \log M)$ BE of the operator $T$, where $\beta \equiv \sum_{i=0}^{M-1} \| \beta_i \|$.
    The gate complexity is given by $\OO(M \log M)$ elementary gates.
\end{lemma}
\begin{proof}
    The proof of this Lemma can be found in many textbooks, see for example~\cite{Lin:2022vrd}.
    %
    The asymptotic cost stems from the complexity of implementing the $\SELECT$ subroutine, since the cost of preparing an arbitrary state on $\log_2 M$ qubits in $\PREPARE$ is $\OO(M)$~\cite{Shende:2006onn,Plesch:2011vwn}, which is cheaper than the cost of $\SELECT$, as we explain next.
    %
    The gate complexity of $\SELECT$ is $\OO(M \log M)$, which comes from sequentially implementing $M$ unitaries, each being controlled on $k=\log M$ ancillary qubits.
    Decomposing $k$-controlled gates into elementary gates can be achieved at a cost linear in $k$, with the constant prefactor being smallest if $k$ additional ancillary qubits are allowed to be used~\cite{Nielsen:2012yss,Babbush:2018ywg}.
    %
    For applications considered in this work, this gives a minor overhead in the qubit cost since $k$ is logarithmic is the parameters of the system.
\end{proof}

Given a BE of the Hamiltonian, one can obtain an approximation to the time evolution operator using QSP.
\begin{theorem}
[QSP with Qubitization]
\label{thm:qspwq}
Let $U_H$ be a an $(\alpha,k)$-block-encoding of a Hamiltonian $H$ acting on a Hilbert space $\mathcal H_s$.
%
Furthermore, let $t$ and $\eps$ be positive real values. 
%
Then there is a quantum circuit that produces a $\left(1 \pm \mathcal O(\eps),k+2\right)$-block-encoding of the time evolution operator $\me^{-iHt}$ up to exponentiation error $\eps$, and possesses a complexity of \begin{equation} \OO\!\left(\alpha t + \log(1/\eps)\right), \end{equation} relative to the oracle $U_H$.
%
The probability for this BE to succeed is
\begin{align}
    p > 1 - \OO(\varepsilon)\,.
\end{align}
\end{theorem}
\begin{proof}
We will not prove this result rigorously, but point the reader to the pedagogical sections of this paper, with all statements made there having been rigorously proved in the literature~\cite{Low:2016znh}. 
%
The fact that the BE is $(\tilde \alpha,\tilde k) = (1 \pm \mathcal O(\eps),k+2)$ can be easily understood.
%
First, the BE of the time evolution operator requires two additional qubits, one ($\sket{q}$) for the qubitization and one ($\sket{b}$) to add the functional dependence on $\phi$, giving $\tilde k = k+2$.
%
The fact that $\tilde \alpha = 1 \pm \mathcal O(\varepsilon)$ follows from the fact that the operator we are block-encoding is a unitary operator, and our approximation is good up to error $\varepsilon$. Since the norm of a unitary operator is 1, this gives that both $\tilde \alpha$ and the success probability are unity (up to $\OO(\varepsilon)$). 
%
\end{proof}

\subsubsection{HHKL}

\begin{theorem}
[HHKL Algorithm]
\label{thm:hhkl_helper}
Let $\Lambda$ be a lattice of qubits embedded in $\dims$-dimensional Euclidean space of size $L$ in each dimension, and let $\hat H$ be a geometrically-local Hamiltonian, normalized such that each local term has norm of order unity. 
%
Further, let $\tilde{t}$ and $\eps$ be positive real values. 
%
Then there exists an algorithm that approximates $\me^{-i\tilde{H}\tilde{t}}$ to exponentiation error $\varepsilon$, which requires\footnote{We assume that the error $\eps$ large enough that the number of calls to the helper function is larger than one.}
\begin{align}
\label{eq:HHKL_calls}
    \OO\!\left( \frac{L^\dims \tilde{t}}{ \log^{\dims}\left(L^\dims \tilde{t}/\eps \right)}\right)
\end{align}
calls to a helper function that implements the time evolution of a system with \MK{size??}
\begin{align}
\label{eq:HHLK_ell_def}
    \ell = \Theta\!\left(\log\left(L^\dims \tilde{t} / \varepsilon\right)\right)
    ,
\end{align}
with error 
\begin{align}
\label{eq:HHLK_delta_def}
    \delta = \OO\!\left( \frac{\varepsilon \log^\dims(L^\dims \tilde{t} / \varepsilon)}{L^\dims \tilde{t}}\right)
\end{align}
\end{theorem}
\begin{proof}
    The results follow directly from our discussion in ~\cref{sec:hhkl}.
    For formal proofs of the results stated there we refer the reader to the original paper~\cite{Haah:2018ekc}.
\end{proof}



\subsubsection{QETU}
\begin{theorem}[QETU]\label{thm:qetu}
Let $U = \me^{-i \tau A}$ with an $n$-qubit Hermitian matrix $A$ and real parameter $\tau$. 
For any real even polynomial $F(x)$ with degree $d$ satisfying $|F(x)| \leq 1, \forall x \in [-1,1]$, one can find a sequence of symmetric phase factors $(\varphi_0, \varphi_1, \dots, \varphi_1, \varphi_0) \in \mathbb{R}^{d+1}$ such that the circuit in~\cref{fig:qetu_circ} denoted by $\mathcal{U}$ satisfies $(\sbra{0} \otimes \unit) \mathcal{U} (\sket{0} \otimes \unit) = F(\cos(\tau A / 2))$. 
\end{theorem}

\begin{proof}
    The proof of the QETU theorem can be found in Appendix~B of Ref.~\cite{Dong:2022mmq}.
\end{proof}


==> tikzlibraryquantikz2.code.tex <==
%This is the quantikz library for typesetting quantum circuits using LaTeX/Tikz. version 1.0.1
% Written by Alastair Kay, 2018. Published under a CC-BY-4.0 licence
% Please email me (alastair.kay@rhul.ac.uk) with any bug reports or feature requests.
% If you find this library useful, please cite its usage in your work, using arXiv:1809.03842, and possibly the DOI: 10.17637/rh.7000520.
% Usage is at your own risk.

%version 1.0.1
% the lstick/midstick/rstick commands now correctly resize braces if you're using classical wires based on wire types at the *end* of each wire (so rstick more likely to look good than lstick/midstick!.
% fixed incompatibility if physics2 package (turned out we both used the same variable name somewhere)
%version 1.0.0
%major new revision with massive under-the-hood changes in how wires work.
%aiming to reduce technical debt in the code as well.
%use the \wire commands for all your wire needs
%fix wire types using wire types={} key, and function setwiretype{}
%check your circuits for places where you assumed there would be no wire.
%some minor changes in optional parameters (e.g. \meter). In practice, these are rarely used, and unlikely to be an issue.
%should always use quantikz and not tikzcd environment

%\ProvidesPackage{quantikz}[2023/05/24 typeset quantum circuit diagrams]

% Package(s) to include
\RequirePackage{xargs,ifthen,xstring,xparse,etoolbox,mathtools,pgfmath}
\RequirePackage{environ} %in an attempt to help with compatibility with the external library of tikz.
%\RequirePackage{tikz}
\usetikzlibrary{cd,decorations.pathreplacing,calc,positioning,fit,shapes.symbols,decorations.pathmorphing,shapes.misc,decorations.markings,math}
\pgfdeclarelayer{background}
\pgfdeclarelayer{quantback}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%create the new quantikz environment
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%I need this to facilitate the external library
%solution taken from https://tex.stackexchange.com/questions/171931/are-the-tikz-libraries-cd-and-external-incompatible-with-one-another
%this does a global redefinition of the &. This is not good as it will lead to incompatibilities with other packages.
%there seems to be a solution https://tex.stackexchange.com/a/633066/148934
%another option, more similar to the original: https://tex.stackexchange.com/a/619983/148934
% \newcommand{\mytikzcdcontext}[2]{
%       \begin{tikzcd}[#1]
%         #2
%       \end{tikzcd}%
% }
%could I do this to align instead?
% \NewDocumentEnvironment{quantikz}{O{}+b}{%
%   \begingroup \catcode`&=\active
%   \def\@temp{\tikzcd@[#1]\scantokens{#2}}%
%   \expandafter\@temp\endtikzcd\endgroup
% }{}
%full solution suggested here https://tex.stackexchange.com/a/682872/148934
\ExplSyntaxOn
\NewDocumentEnvironment{quantikz}{O{}+b}{
\gdef\toslice@qtkz{0}\def\vert@qtkz{0}%
  \begin{tikzpicture}[/tikz/commutative~diagrams/.cd, every~diagram,baseline={([yshift=-axis_height]\tikzcdmatrixname)}, #1]
  \pgfsetlayers{background,quantback,main}
    \tl_set:Nn \l_tmpa_tl { #2 }
    \tl_replace_all:Nnn \l_tmpa_tl { & } { \pgfmatrixnextcell }
    \begingroup%doing it like this, we don't need to patch tikzcd, so it will continue to work independently.
      \def\tikzpicture[##1]{}
      \let\endtikzpicture\relax
      \tikzcd[#1]
        \l_tmpa_tl
      \endtikzcd
    \endgroup
  \end{tikzpicture}
}{}
\ExplSyntaxOff

% \ExplSyntaxOn
% \NewDocumentEnvironment{quantikz}{O{}+b}{%
%   \tl_rescan:nn { \char_set_catcode_active:N \& } { \begin{tikzcd}[#1] #2 \end{tikzcd} }
% }{}
% \ExplSyntaxOff

% \newcommand{\mytikzcdcontext}[2]{
%   \begin{tikzpicture}[baseline=(maintikzcdnode.base)]
%     \node (maintikzcdnode) [inner sep=0, outer sep=0] {%
%       \begin{tikzcd}[#1]
%         #2
%       \end{tikzcd}%
%     };
%   \end{tikzpicture}%
% }

% \ExplSyntaxOn

% \NewDocumentEnvironment{quantikz}{O{}+b}
%  {
%   \tl_set:Nn \l_tmpa_tl { #2 }
%   \regex_replace_all:nnN { \& } { \cA\& } \l_tmpa_tl
%   \weird_wonderful_mytikzcd:nV { #1 } \l_tmpa_tl
%  }
%  {}

% \cs_set_eq:NN \weird_wonderful_mytikzcd:nn \mytikzcdcontext
% \cs_generate_variant:Nn \weird_wonderful_mytikzcd:nn { nV }

% \ExplSyntaxOff


%patch tikzcd to allow for multiple layers of commands that get deferred until later
% \patchcmd\tikzcd@{\tikzpicture}{%
%   \def\toslice{0}\def\vert@qtkz{0}%
%  \begin{tikzpicture}}{}{}
%\patchcmd\tikzcd@{\tikzpicture[/tikz/commutative diagrams/.cd,every diagram,#1]}{%
%}{}{}
\patchcmd\tikzcd@
    {\global\let\tikzcd@savedpaths\pgfutil@empty}
    {\global\let\tikzcd@savedpaths\pgfutil@empty
    \pgfutil@g@addto@macro\tikzcd@savedpaths{\begin{scope}[/tikz/commutative diagrams/.cd,#1]}
    \pgfsetlayers{background,quantback,main}
    \global\let\tikzcd@atendsavedpaths\pgfutil@empty
    \global\let\tikzcd@atendlabels\pgfutil@empty
    \global\let\tikzcd@atendslices\pgfutil@empty
    \pgfutil@g@addto@macro\tikzcd@savedpaths\DivideRowsCols
    \def\tikz@lib@matrix@empty@cell{
      \iftikz@lib@matrix@empty\node[name=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn,
      minimum width=\ifcsundef{cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}{0}{\csname cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn\endcsname},
      minimum height=\ifcsundef{cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}{0}{\csname cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn\endcsname}
      ]{};\wire{a}\fi
      \csgundef{cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      \csgundef{cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}}
    %\pgfmathsetmacro{\mname}{random(100000)}
    \ifcsstring{toslice@qtkz}{1}{\ifcsstring{vert@qtkz}{0}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}
    %\ifthenelse{\toslice=1}{\ifthenelse{\vert@qtkz=0}{\PackageWarning{quantikz}{We are slicing}\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}
    }{}{}

%this patching works on modern systems, but I believe is incompatible with the old version that arXiv is running
%\patchcmd\endtikzcd{\tikzcd@savedpaths}{\tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices}{}{}

%instead, completely redefine the function
\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \begin{pgfonlayer}{quantback}
    \begingroup
    \tikzcdset{wire types/.code={}}%prevent setting of wire types, which wipes all the work we've done!
    %\begin{scope} already included in tikzcd@savedpaths so that it has right options
      \tikzcd@savedpaths
    \end{scope}
    \endgroup
    \end{pgfonlayer}
    \tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices%I just added stuff here instead
    \resetwiretypes%reset wire types
    \def\tikz@lib@matrix@empty@cell{\iftikz@lib@matrix@empty\node[name=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn]{};\fi}%
  \endgroup%
  \endtikzpicture%
  \ifnum0=`{}\fi}


%end patching


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% the basic wire command
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ExplSyntaxOn
% take a direction, such as d and repeat it the required number of times
\NewExpandableDocumentCommand{\myrepeat}{O{}mm}
 {
  \int_compare:nT { #2 > 0 }
   {
    #3 \prg_replicate:nn { #2 - 1 } { #1#3 }
   }
 }
\ExplSyntaxOff

%this is the main entry point for people
%converts a wire command with distance into one using repeated letters (main directions only)
\NewDocumentCommand{\wire}{O{l}O{1}O{}m}{%direction (l/r/u/d), distance, decoration, quantum/classical/bundle/none
\ifstrequal{#2}{0}{%
\PackageWarning{quantikz}{You seem to have a wire of zero length. I believe the problem is in cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}.
}{%
  \edef\length{\myrepeat{#2}{#1}}
\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{%
\expandafter\fullwire\expandafter{\length}{#1}{#4}{#3}%
}{}
}}
%does the actual business of creating the different wire types with the correct anchors
%uses custom anchors on shapes for classical wires. We'll come to this in a minute.
\newcommand{\fullwire}[4]{%direction with repetition. direction. type. decoration
\edef\wiretype{#3}
\ifstrequal{#3}{a}{%automatic determination
  \ifcsundef{wire@type@\the\pgfmatrixcurrentrow}{%type not defined globally. assume quantum.
  \edef\wiretype{q}
  }{%
  \edef\wiretype{\csname wire@type@\the\pgfmatrixcurrentrow\endcsname}
  \ifdefstring{\wiretype}{u}{%
    \edef\wiretype{q}
  }{}
  }
  \ifcsdef{wire@type@override@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}{%
    \edef\wiretype{\csname wire@type@override@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn\endcsname}
  }{}
}{}
\ifdefstring{\wiretype}{q}{%quantum wire
    \arrow[#1,arrows,#4] {}
  }{%
  \ifdefstring{\wiretype}{c}{%classical wire
    \arrow[arrows,start anchor=#2startone,end anchor=#2endone] {#1}\arrow[arrows,start anchor=#2starttwo,end anchor=#2endtwo,#4] {#1}
  }{%
  \ifdefstring{\wiretype}{b}{%wire bundle
    \arrow[arrows,start anchor=#2startone,end anchor=#2endone,#4] {#1}\arrow[arrows,start anchor=#2starttwo,end anchor=#2endtwo,#4] {#1}\arrow[#1,arrows,#4] {}
  }{%
  \ifdefstring{\wiretype}{n}{%no wire
  }{\ifdefstring{\wiretype}{u}{%unset
  }{\PackageWarning{quantikz}{unknown wire type in cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}}}}}}
}

\newcommand{\setwiretype}[2][\the\pgfmatrixcurrentrow]{%
%this command will record what the current wire type is supposed to be
\ifstrequal{#2}{u}{
  \csgundef{wire@type@#1}
}{
\expandafter\gdef\csname wire@type@#1\endcsname{#2}%will need to reset all these variables at the beginning/end of a circuit.
}
}

\NewDocumentCommand{\wireoverride}{O{\the\pgfmatrixcurrentrow}O{\the\pgfmatrixcurrentcolumn}m}{%
%change the wire type of this specific cell without unsetting the global wire type of this cell.
\expandafter\gdef\csname wire@type@override@#1-#2\endcsname{#3}
}

\newcounter{dummy}
\newcommand{\importwiretypes}[1]{%
%receive a list of wire types. Process them into individual variables
\setcounter{dummy}{1}% 
  \foreach \thiswire [count=\rownum] in {#1} {%
    \expandafter\expandafter\expandafter\setwiretype\expandafter\expandafter\expandafter[\expandafter\rownum\expandafter]\expandafter{\thiswire}
    \stepcounter{dummy}
     }
     \pgfmathparse{\arabic{dummy}/2}
     %\pgfmathresult
     \expandafter\setmiddle\expandafter{\pgfmathresult}
  }%

\newcommand{\resetwiretypes}{%try to reset all definitions of per-row wire types
  \foreach \rownum in {1,...,\the\pgfmatrixcurrentrow} {%
\expandafter\setwiretype\expandafter[\rownum]{u} 
  }
}

\tikzset{%
  strike arrow/.style n args={3}{
    decoration={markings, mark=at position 0.5 with {
        \draw [internal,-] 
            ++ (#1, #2 )
            -- ( -#1, -#2) node [anchor=south west, inner sep=0pt] {$\scriptstyle #3$};} %can I use pgfkeys and do some maths here?
    },
    postaction={decorate},
}}
%this used to be a more complex command, but is now only used for adding the strikethrough + number
\newcommand{\qwbundle}[2][]{%
		%\ifthenelse{\the\pgfmatrixcurrentcolumn=2}{%do the strikethrough
  \pgfkeys{/quantikz/gates/.cd,style=,Strike Width=0.08cm,Strike Height=0.12cm,#1} 
  \pgfkeysgetvalue{/quantikz/gates/style}{\style}
  \pgfkeysgetvalue{/quantikz/gates/Strike Width}{\sw}
  \pgfkeysgetvalue{/quantikz/gates/Strike Height}{\sh}
  \edef\arg{strike arrow={\sw}{\sh}{#2},\style}
			\expandafter\arrow\expandafter[\arg,phantom]{l}%
	}

%%%%%%%%%%%%%%%%%%%%%%%%%
%
% deprecated wire commands provided for backwards compatibility
%
%%%%%%%%%%%%%%%%%%%%%%%%%


%now add some of the basic wire commands for backwards compatibility. These should be largely superfluous once I'm done.
\newcommand{\vcw}[1]{%vertical classical wire. goes down by the amount specified in arg
\ifnumcomp{#1}{>}{0}{%
  \wire[d][#1]{c}
}{\ifnumcomp{#1}{<}{0}{%
  \wire[u][-#1]{c}
}{\PackageWarning{quantikz}{You seem to have a vertical classical wire with no height in cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn!}}}
}
%vertical quantum wire, relative positioning
\newcommand{\vqw}[1]{
\ifnumcomp{#1}{>}{0}{%
  \wire[d][#1]{q}
}{\ifnumcomp{#1}{<}{0}{%
  \wire[u][-#1]{q}
}{\PackageWarning{quantikz}{You seem to have a vertical quantum wire with no height in cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn!}}}
}

%basic horzontal quantum wire, length 1. Goes backwards 1 cell. Won't do anything in the first cell.
\newcommand{\qw}{\wire{q}}
%basic horzontal classical wire, length 1. Goes backwards 1 cell. Won't do anything in the first cell.
\newcommand{\cw}{\wire{c}}
%use for fudging classical wires that have horizontal and vertical sections
%shouldn't really be necessary any more?
\NewExpandableDocumentCommand{\cwbend}{m}{
  \phase{}\vcw{#1}\cw
  % \edef\cell{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
  % \expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
  %   \expandafter\latephase@end\expandafter{\cell}
  % }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% shape definitions
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%we will mainly be using rectangle and circle as base shapes. Also signal, rounded rectangle for some measurement objects. cross out for swap.
%First we need to add custom anchors to them for attaching the wires.

%helper functions
\newcommand*\pgfdeclareanchoralias[3]{%
    \expandafter\def\csname pgf@anchor@#1@#3\expandafter\endcsname
            \expandafter{\csname pgf@anchor@#1@#2\endcsname}}
\def\pgfaddtoshape#1#2{%
  \begingroup
  \def\pgf@sm@shape@name{#1}%
  \let\anchor\pgf@sh@anchor
  #2%
  \endgroup
}

%add anchors to the rectangle
\pgfaddtoshape{rectangle}{%
    \anchor{dendtwo}{%
    \pgf@process{\southwest}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@x by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%
  \anchor{dstarttwo}{%
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@x by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%
  \anchor{dendone}{%
    \pgf@process{\southwest}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@x by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%
  \anchor{dstartone}{%
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@x by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%
    \anchor{lstarttwo}{%
    \pgf@process{\northeast}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
    \advance\pgf@y by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%
  \anchor{lendtwo}{%
    \pgf@process{\southwest}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\northeast}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
    \advance\pgf@y by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%
  \anchor{lstartone}{%
    \pgf@process{\northeast}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
    \advance\pgf@y by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%
  \anchor{lendone}{%
    \pgf@process{\southwest}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\northeast}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
    \advance\pgf@y by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%
  }
\pgfdeclareanchoralias{rectangle}{dendtwo}{ustarttwo}
\pgfdeclareanchoralias{rectangle}{dendone}{ustartone}
\pgfdeclareanchoralias{rectangle}{dstarttwo}{uendtwo}
\pgfdeclareanchoralias{rectangle}{dstartone}{uendone}
\pgfdeclareanchoralias{rectangle}{lendtwo}{rstarttwo}
\pgfdeclareanchoralias{rectangle}{lendone}{rstartone}
\pgfdeclareanchoralias{rectangle}{lstarttwo}{rendtwo}
\pgfdeclareanchoralias{rectangle}{lstartone}{rendone}

%add anchors to the circle
\pgfaddtoshape{circle}{%
  \anchor{dstartone}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap=" key to a value smaller than 0.06cm.}
    }{}
    \pgfmathparse{-sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})}
    \advance\pgf@y by\pgfmathresult pt
  }%
  \anchor{dstarttwo}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@x by\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}
    \pgfmathparse{-sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})}
    \advance\pgf@y by\pgfmathresult pt
  }%
  \anchor{dendone}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@x by-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}
    \pgfmathparse{sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})}
    \advance\pgf@y by\pgfmathresult pt
  }%
  \anchor{dendtwo}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@x by\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}
    \pgfmathparse{sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})}
    \advance\pgf@y by\pgfmathresult pt
  }%
  \anchor{lstartone}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@y by-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}
    \pgfmathparse{-sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})}
    \advance\pgf@x by\pgfmathresult pt
  }%
  \anchor{lstarttwo}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@y by\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}
    \pgfmathparse{-sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})}
    \advance\pgf@x by\pgfmathresult pt
  }%
  \anchor{lendone}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@y by-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}
    \pgfmathparse{sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})}
    \advance\pgf@x by\pgfmathresult pt
  }%
  \anchor{lendtwo}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@y by\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}
    \pgfmathparse{sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})}
    \advance\pgf@x by\pgfmathresult pt
  }%
}
\pgfdeclareanchoralias{circle}{dendtwo}{ustarttwo}
\pgfdeclareanchoralias{circle}{dendone}{ustartone}
\pgfdeclareanchoralias{circle}{dstarttwo}{uendtwo}
\pgfdeclareanchoralias{circle}{dstartone}{uendone}
\pgfdeclareanchoralias{circle}{lendtwo}{rstarttwo}
\pgfdeclareanchoralias{circle}{lendone}{rstartone}
\pgfdeclareanchoralias{circle}{lstarttwo}{rendtwo}
\pgfdeclareanchoralias{circle}{lstartone}{rendone}

\pgfaddtoshape{rounded rectangle}{%
%I'm going to cheat and assume it's always wide enough to have a flat bottom/top.
	\anchor{dstartone}{%
 		\roundedrectanglepoints%
 		\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{-\halfheight-\outerysep}}%
	}
	\anchor{dstarttwo}{%
 		\roundedrectanglepoints%
 		\pgfpointadd{\centerpoint}{\pgfpoint{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{-\halfheight-\outerysep}}%
	}
	\anchor{dendone}{%
 		\roundedrectanglepoints%
 		\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{\halfheight+\outerysep}}%
	}
	\anchor{dendtwo}{%
 		\roundedrectanglepoints%
 		\pgfpointadd{\centerpoint}{\pgfpoint{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{\halfheight+\outerysep}}%
	}
	\anchor{lstarttwo}{%
	\roundedrectanglepoints%
    \ifx\westarc\pgf@lib@sh@misc@rr@text@concave%
    %not sure! Just leave it. I don't think even the simple quantum wire works as I want it out the box!
    \pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\outerxsep}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}%
        % \pgfpathlineto{\pgfpoint{-\halfwidth-\arcwidth}{+-\halfheight}}%
        % \pgfpatharc{+-\halfarcangle}{+\halfarcangle}{+\radius}%
    \else%
        \ifx\westarc\pgf@lib@sh@misc@rr@text@convex%
        		\pgfextract@process\arccenter{%
               	\pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\chordwidth+\radius}{+0pt}}%
            }%
            \pgfmathparse{sqrt((\radius+\outerxsep)^2-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}^2)}
            \pgfpointadd{\arccenter}{\pgfpoint{-\pgfmathresult pt}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}
        \else%
            \pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\outerxsep}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}%
        \fi%
    \fi%
	}
	\anchor{lstartone}{%
	\roundedrectanglepoints%
   \ifx\westarc\pgf@lib@sh@misc@rr@text@concave%
    %not sure!
    \pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\outerxsep}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}%
    %     % \pgfpathlineto{\pgfpoint{-\halfwidth-\arcwidth}{+-\halfheight}}%
    %     % \pgfpatharc{+-\halfarcangle}{+\halfarcangle}{+\radius}%
    \else%
        \ifx\westarc\pgf@lib@sh@misc@rr@text@convex%
        		\pgfextract@process\arccenter{%
               	\pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\chordwidth+\radius}{+0pt}}%
            }%
            \pgfmathparse{sqrt((\radius+\outerxsep)^2-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}^2)}
            \pgfpointadd{\arccenter}{\pgfpoint{-\pgfmathresult pt}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}
        \else%
            \pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\outerxsep}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}%
        \fi%
    \fi%
	}	
	\anchor{lendtwo}{%
	\roundedrectanglepoints%
    \ifx\eastarc\pgf@lib@sh@misc@rr@text@concave%
    %not sure!
        % \pgfpathlineto{\pgfpoint{-\halfwidth-\arcwidth}{+-\halfheight}}%
        % \pgfpatharc{+-\halfarcangle}{+\halfarcangle}{+\radius}%
    \else%
        \ifx\eastarc\pgf@lib@sh@misc@rr@text@convex%
        		\pgfextract@process\arccenter{%
               	\pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth+\chordwidth-\radius}{+0pt}}%
            }%
            \pgfmathparse{sqrt((\radius+\outerxsep)^2-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}^2)}
            \pgfpointadd{\arccenter}{\pgfpoint{\pgfmathresult pt}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}
            %\pgfpathlineto{\pgfpoint{-\halfwidth-\chordwidth+\arcwidth}{+-\halfheight}}%
            %\pgfpatharc{180+\halfarcangle}{180-\halfarcangle}{+\radius}%
        \else%
            \pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}%
        \fi%
    \fi%
	}
	\anchor{lendone}{%
	\roundedrectanglepoints%
    \ifx\eastarc\pgf@lib@sh@misc@rr@text@concave%
    %not sure!
        % \pgfpathlineto{\pgfpoint{-\halfwidth-\arcwidth}{+-\halfheight}}%
        % \pgfpatharc{+-\halfarcangle}{+\halfarcangle}{+\radius}%
    \else%
        \ifx\eastarc\pgf@lib@sh@misc@rr@text@convex%
        		\pgfextract@process\arccenter{%
               	\pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth+\chordwidth-\radius}{+0pt}}%
            }%
            \pgfmathparse{sqrt((\radius+\outerxsep)^2-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}^2)}
            \pgfpointadd{\arccenter}{\pgfpoint{\pgfmathresult pt}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}
            %\pgfpathlineto{\pgfpoint{-\halfwidth-\chordwidth+\arcwidth}{+-\halfheight}}%
            %\pgfpatharc{180+\halfarcangle}{180-\halfarcangle}{+\radius}%
        \else%
            \pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}%
        \fi%
    \fi%
	}
	}
\pgfdeclareanchoralias{rounded rectangle}{dendtwo}{ustarttwo}
\pgfdeclareanchoralias{rounded rectangle}{dendone}{ustartone}
\pgfdeclareanchoralias{rounded rectangle}{dstarttwo}{uendtwo}
\pgfdeclareanchoralias{rounded rectangle}{dstartone}{uendone}
\pgfdeclareanchoralias{rounded rectangle}{lendtwo}{rstarttwo}
\pgfdeclareanchoralias{rounded rectangle}{lendone}{rstartone}
\pgfdeclareanchoralias{rounded rectangle}{lstarttwo}{rendtwo}
\pgfdeclareanchoralias{rounded rectangle}{lstartone}{rendone}


\pgfaddtoshape{signal}{%
	\anchor{lstarttwo}{%
		\installsignalparameters
		\let\firstpoint\anchornorthwest
		\let\secondpoint\anchorwest
    \pgfpointintersectionoflines%
      {\firstpoint}%
      {\secondpoint}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0cm}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0.5cm}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}}%
	}
	\anchor{lstartone}{%
		\installsignalparameters
		\let\firstpoint\anchorsouthwest
		\let\secondpoint\anchorwest
		\pgfpointintersectionoflines%
      {\firstpoint}%
      {\secondpoint}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0cm}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0.5cm}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}}%
	}
	\anchor{lendtwo}{%
		\installsignalparameters
		\let\firstpoint\anchornortheast
		\let\secondpoint\anchoreast
    \pgfpointintersectionoflines%
      {\firstpoint}%
      {\secondpoint}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0cm}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0.5cm}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}}%
	}
	\anchor{lendone}{%
		\installsignalparameters
		\let\firstpoint\anchorsoutheast
		\let\secondpoint\anchoreast
    \pgfpointintersectionoflines%
      {\firstpoint}%
      {\secondpoint}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0cm}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0.5cm}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}}}%
	}
  \anchor{dstarttwo}{%
  	\installsignalparameters
    \pgf@process{\southanchor}%
    \advance\pgf@x by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%
  \anchor{dstartone}{%
  	\installsignalparameters
    \pgf@process{\southanchor}%
    \advance\pgf@x by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%
  \anchor{dendtwo}{%
  	\installsignalparameters
    \pgf@process{\northanchor}%
    \advance\pgf@x by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%
  \anchor{dendone}{%
  	\installsignalparameters
    \pgf@process{\northanchor}%
    \advance\pgf@x by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}%
  }%}
 }
\pgfdeclareanchoralias{signal}{dendtwo}{ustarttwo}
\pgfdeclareanchoralias{signal}{dendone}{ustartone}
\pgfdeclareanchoralias{signal}{dstarttwo}{uendtwo}
\pgfdeclareanchoralias{signal}{dstartone}{uendone}
\pgfdeclareanchoralias{signal}{lendtwo}{rstarttwo}
\pgfdeclareanchoralias{signal}{lendone}{rstartone}
\pgfdeclareanchoralias{signal}{lstarttwo}{rendtwo}
\pgfdeclareanchoralias{signal}{lstartone}{rendone}

% if these base shapes won't do, you'll have to create your own definition, either of a whole shape or take an existing one and add extra anchors, as above.
% you need to make sure that the anchor border works correctly for lines approaching from the 4 compass points, as these are where the quantum wires attach.
% classical wires instead attach to points that are displaced by a horizontal/vertical amount \pgfkeysvalueof{/tikz/commutative diagrams/classical gap} relative to these positions. These are called:
% dstartone,dstarttwo,dendone,dendtwo
% ustartone,ustarttwo,uendone,uendtwo
% lstartone,lstarttwo,lendone,lendtwo
% rstartone,rstarttwo,rendone,rendtwo
%The idea, for example, is if you have an "l" type classical wire, there will be two wires, one going from lstartone (the left-hand edge on your shape, \pgfkeysvalueof{/tikz/commutative diagrams/classical gap} vertically above the west anchor) and going to lendone (l end one) on the cell one to the left. Typically, you expect lendone and rstartone to be the same points. There is also a line from lstarttwo to lendtwo.

% often the shape you want can just be a modification of an existing shape. Critically, the border should be the same. Then we don't need to define a whole new shape, we can just do it with styles. Much easier!

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% gate definitions
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%single qubit operations
%\tikzset{linecont/.style={line}}
\newcommand{\phantomgate}[1]{|[line,thickness, inner ysep=3pt]| \phantom{#1}}
\newcommand{\hphantomgate}[1]{|[line,minimum size=1.5em,thickness]| \hphantom{#1}}
\newcommand{\linethrough}{|[line,thickness, inner ysep=3pt]| }
\newcommand{\push}[1]{#1}
%\newcommand{\alias}[1]{|[alias=#1]|}

\tikzset{
circle phase/.style={fill,shape=circle,minimum size=0.12cm,draw},
rrectangle phase/.style={fill,shape=rectangle,rounded corners=1.5pt,minimum width=3pt,minimum height=2.5*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}+3pt,draw},
phase/.code={%
  \pgfkeys{/quantikz/gates/.cd,style=,label style=,#1}%
  \pgfkeysgetvalue{/quantikz/gates/style}{\style}
  \ifcsundef{wire@type@\the\pgfmatrixcurrentrow}{%type not defined globally. assume quantum.
    \edef\wiretype{q}
  }{%
    \edef\wiretype{\csname wire@type@\the\pgfmatrixcurrentrow\endcsname}
  }
  \ifcsstring{wiretype}{b}{\ifdimless{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{0.04cm}{\tikzset{circle phase}}{\tikzset{rrectangle phase}}}{%
    \ifcsstring{wiretype}{c}{\ifdimless{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}{0.04cm}{\tikzset{circle phase}}{\tikzset{rrectangle phase}}}{\tikzset{circle phase}}
  }
  \expandafter\tikzset\expandafter{\style}
  \pgfkeys{/quantikz/gates/.cd,style=,label style=,#1}%run again so that "open" can take priority
  },
%ophase/.style={fill=\pgfkeysvalueof{/tikz/commutative diagrams/background color},draw,shape=circle,minimum size=3*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}
phase label/.code={\tikzset{label distance=2mm,anchor=mid,label position=45}
  \pgfkeys{/quantikz/gates/.cd,style=,label style=,#1}%
  \pgfkeysgetvalue{/quantikz/gates/style}{\tstyle}
  \pgfkeysgetvalue{/quantikz/gates/label style}{\lstyle}
  \edef\style{\tstyle,\lstyle}
  \expandafter\tikzset\expandafter{\style}
},
}

\DeclareExpandableDocumentCommand{\phase}{O{}m}{|[phase={#1},label={[phase label={#1}]#2}]| {}}
\DeclareExpandableDocumentCommand{\control}{O{}m}{|[phase={#1}]| {}}
\DeclareExpandableDocumentCommand{\ocontrol}{O{}m}{|[phase={#1,open}]| {}}
\DeclareExpandableDocumentCommand{\targ}{O{}m}{|[circlewc={#1}]| {}}
\DeclareExpandableDocumentCommand{\targX}{O{}m}{|[crossx2={#1}]| {}}


\tikzset{
	cross/.style={path picture={ 
		\draw[internal](path picture bounding box.north) -- (path picture bounding box.south) (path picture bounding box.west) -- (path picture bounding box.east);
	}},
  circlewc/.code={
  \tikzset{draw,circle,cross,minimum width=4pt,inner sep=3pt}
    \pgfkeys{/quantikz/gates/.cd,style=,#1}%
    \pgfkeysgetvalue{/quantikz/gates/style}{\style}
    \expandafter\tikzset\expandafter{\style}
  },
  crossx/.style={path picture={ 
		\draw[internal,inner sep=0pt]
		(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east); %(path picture bounding box.west) -- (path picture bounding box.east);
	}},
  crossdraw/.pic = {
    \begin{pgfinterruptboundingbox}
      \node[cross out,draw,minimum size=0.7em,#1] {};
    \end{pgfinterruptboundingbox}
  },
  crossx2/.code={
    \pgfkeys{/quantikz/gates/.cd,style=,#1}%
    \pgfkeysgetvalue{/quantikz/gates/style}{\style}
    \edef\styling{crossx3=\style}
    \expandafter\tikzset\expandafter{\styling}
  },
  crossx3/.style={
    append after command={
      (\tikzlastnode.center) pic{crossdraw={#1}}
    }
  }
}

%%%
%
%measuring
%
%%%

%standard meter device
%first, define the styles
\tikzset{
  meter/.style={draw,
    %fill=\pgfkeysvalueof{/tikz/commutative diagrams/background color},
    filling,
    minimum width=2em,
    minimum height=1.5em,
    rectangle, 
    font=\vphantom{A}, 
    thickness,
    path picture={
        \draw ([shift={(.1,-.06)}]path picture bounding box.west) to[bend left=50] ([shift={(-.1,-.06)}]path picture bounding box.east);
        \draw[-{Latex[scale=0.6]}] ([shift={(0,-.1)}]path picture bounding box.center) -- ([shift={(-.1,.2)}]path picture bounding box.east);
    },
    },
    my label/.style={yshift=0.1cm,above,align=center},
}
%\DeclareExpandableDocumentCommand{\meter}{O{}{m}}{|[meter,label={[my label]#2},#1]| {}}
% \DeclareExpandableDocumentCommand{\meter}{O{}O{1.5pt}O{1.5pt}m}{%
% \gate[priority label={above},priority style={meter},#1][#2][#3]{#4}
% }
\DeclareExpandableDocumentCommand{\meter}{O{}O{2em}O{1.5em}m}{%
\gate[#1,priority label=above,ps=meter,disable auto height][#2][#3]{#4}
}
%code not working here :( Either I can get my predefined label style to apply, or the user's custom style. Not both.

%gate variant with classical result wire
\tikzset{
    metercw/.style={draw=none,
    yshift=0.375em,
        fill=none,
        minimum width=2em,
        minimum height=2.25em,
        font=\vphantom{A}, 
        thickness,
        path picture={
        %if you draw the rectangle to be the full width of the box, you cut off half the line, so have to bring it in a little.
        \node[draw,thickness,filling,#1,inner sep=0pt, minimum height=0pt,minimum width=0pt,fit={([shift={(.5\pgflinewidth,.5\pgflinewidth)}]path picture bounding box.south west) ([shift={(-.5\pgflinewidth,-0.75em)}]path picture bounding box.north east)}] (rect) {};
        %  \draw [#1]([xshift={0.5\pgflinewidth}]path picture bounding box.south west) rectangle ([yshift=-0.75em,xshift={-0.5\pgflinewidth}]path picture bounding box.north east);
          %draw the two classical wires
          \draw ([xshift=\pgfkeysvalueof{/tikz/commutative diagrams/classical gap},yshift=-0.75em]path picture bounding box.north) -- ([xshift=\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}]path picture bounding box.north);
          \draw ([xshift=-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap},yshift=-0.75em]path picture bounding box.north) -- ([xshift=-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}]path picture bounding box.north);
          %draw the image in the middle of the box
            \draw ([shift={(.1,-.06)}]rect.west) to[bend left=50] ([shift={(-.1,-.06)}]rect.east);
        \draw[-{Latex[scale=0.6]}] ([shift={(0,-.1)}]rect.center) -- ([shift={(-.1,.2)}]rect.east);
        }
    }
}
%\DeclareExpandableDocumentCommand{\metercw}{O{}{m}}{|[metercw={#1},label={[my labelcw]#2}]| {}}
\DeclareExpandableDocumentCommand{\metercw}{O{}O{2em}O{2.25em}m}{%
\gate[#1,priority label=above,ps=metercw,disable auto height][#2][#3]{#4}
}

\tikzset{measuretab/.style={draw,signal,signal to=west,filling,minimum width=2em, minimum height=1em,inner sep=4pt}}
\DeclareExpandableDocumentCommand{\measuretab}{O{}{m}}{|[measuretab,#1]| {#2}}
%considered making this a multiqubit gate, but any non-straight edge works badly with incoming wires and transparency.
%it might be that your use case is tolerable.
% \DeclareExpandableDocumentCommand{\measuretab}{O{}O{2em}O{1.5pt}m}{%
% \gate[#1,ps=measuretab][#2][#3]{#4}
% }

\tikzset{
  meterD/.style={
        draw,
        shape=rounded rectangle,
        rounded rectangle west arc=none,
        inner sep=4pt,
        filling
    },
  inputD/.style={
        draw,
        shape=rounded rectangle,
        rounded rectangle east arc=none,
        inner sep=4pt,
        filling
    }
}
%should these have a multi-qubit option?
\DeclareExpandableDocumentCommand{\meterD}{O{}{m}}{|[meterD,#1]| {#2}}
\DeclareExpandableDocumentCommand{\inputD}{O{}{m}}{|[inputD,#1]| {#2}\wireoverride{n}}
% \DeclareExpandableDocumentCommand{\meterD}{O{}O{1.5pt}O{1.5pt}m}{%
% \gate[#1,ps=meterD][#2][#3]{#4}
% }
\tikzset{measure/.style={draw=black,rounded rectangle,filling, minimum width=2em, minimum height=1em, inner sep=4pt}}

% \DeclareExpandableDocumentCommand{\measure}{O{}O{2em}O{1.5pt}m}{%
% \gate[#1,ps=measure][#2][#3]{#4}
% }

\DeclareExpandableDocumentCommand{\measure}{O{}{m}}{|[measure,#1]| {#2}}


\tikzset{trash/.style={path picture={
    \edef\yshift{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}
    \ifcsstring{wire@type@\the\pgfmatrixcurrentrow}{c}{%
      \draw[internal,inner sep=0pt,-stealth] ([yshift={\yshift}]path picture bounding box.west) -- ([yshift={\yshift}]path picture bounding box.center) -- (path picture bounding box.south);
      \draw[internal,inner sep=0pt] ([yshift={-\yshift}]path picture bounding box.west) -- ([yshift={-\yshift}]path picture bounding box.center);
    }{%
      \draw[internal,inner sep=0pt,-stealth] (path picture bounding box.west) -- (path picture bounding box.center) -- (path picture bounding box.south);
      \ifcsstring{wire@type@\the\pgfmatrixcurrentrow}{b}{%
        \draw[internal,inner sep=0pt] ([yshift={\yshift}]path picture bounding box.west) -- ([yshift={\yshift}]path picture bounding box.center) -- (path picture bounding box.center);
        \draw[internal,inner sep=0pt] ([yshift={-\yshift}]path picture bounding box.west) -- ([yshift={-\yshift}]path picture bounding box.center);
      }{}
    }
    %\edef\yshift{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}
    },
    minimum height=2.5em,
    minimum width=2em}}

\DeclareExpandableDocumentCommand{\trash}{O{}{m}}{|[trash,label={below:#2},#1]| {}}

\tikzset{ground/.style={path picture={
    \draw[internal,inner sep=0pt]([xshift={0.5\pgflinewidth}]path picture bounding box.south west) -- ([xshift={0.5\pgflinewidth}]path picture bounding box.north west);
    \draw[internal,inner sep=0pt]([xshift={0.5\pgflinewidth+2*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}},yshift={\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}]path picture bounding box.south west) -- ([xshift={0.5\pgflinewidth+2*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}},yshift={-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}]path picture bounding box.north west);
    \draw[internal,inner sep=0pt]([xshift={0.5\pgflinewidth+4*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}},yshift={2*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}]path picture bounding box.south west) -- ([xshift={0.5\pgflinewidth+4*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}},yshift={-2*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}]path picture bounding box.north west);
  },
  minimum height=8*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap},
  minimum width=5*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}
  }}
\DeclareExpandableDocumentCommand{\ground}{O{}{m}}{|[ground,label={below:#2},#1]| {}}
%\DeclareExpandableDocumentCommand{\bin}{O{}{m}}{|[bin,label={below:#2},#1]| {}}

% \def\bin{\begin{tikzpicture}[thickness,scale=0.2]
%\draw (0,0) -- (1,0) -- (1,-0.2) -- (2,-0.8) -- (1.4,-3) -- (-0.4,-3) -- (-1,-0.8) -- (0,-0.2) -- cycle;
% \draw (2,-0.8) arc (360:180:1.5 and 0.2);
% \draw (-0.2,-1.1) -- (0.3,-2.8);
% \draw (1.2,-1.1) -- (0.7,-2.8);
% \end{tikzpicture}}


%%%
%
%controlled gates
%
%%%

\NewExpandableDocumentCommand{\ctrl}{O{}m}{\control[#1]{}%
  \pgfkeys{/quantikz/gates/.cd,style=,label style=,wire style=,vertical wire=q,#1}%
  \pgfkeysgetvalue{/quantikz/gates/style}{\tstyle}
  \pgfkeysgetvalue{/quantikz/gates/wire style}{\wstyle}
  \edef\style{\tstyle,\wstyle}
  \pgfkeysgetvalue{/quantikz/gates/vertical wire}{\wtype}
\ifnumcomp{#2}{>}{0}{%
   \expandafter\expandafter\expandafter\expandedwire\expandafter\expandafter\expandafter{\expandafter\style\expandafter}\expandafter{\wtype}{d}{#2}
% %  \wire[d][#2][\style]{\wtype}
}{}
\ifnumcomp{#2}{<}{0}{%
  \expandafter\expandafter\expandafter\expandedwire\expandafter\expandafter\expandafter{\expandafter\style\expandafter}\expandafter{\wtype}{u}{-#2}
%  \wire[u][-#3][#2]{#1}
}{}
}
\NewExpandableDocumentCommand{\octrl}{O{}m}{\ctrl[#1,open]{#2}}

\NewDocumentCommand\expandedwire{mmmm}{\wire[#3][#4][#1]{#2}}

\DeclareExpandableDocumentCommand{\swap}{O{}m}{%styling,label of partial swap, displacement of partial swap, distance
|[crossx2={#1}]| {}
\pgfkeys{/quantikz/gates/.cd,partial swap=,style=,partial position=0.5,label style=,vertical wire=q,#1}%
\pgfkeysgetvalue{/quantikz/gates/partial swap}{\partial}
\pgfkeysgetvalue{/quantikz/gates/vertical wire}{\wtype}
\pgfkeysgetvalue{/quantikz/gates/style}{\tstyle}
\ifdefempty{\partial}{%
  \edef\tempstyle{\tstyle}
%   \expandafter\vqw\expandafter[\opts]{#2}
  }{%
%   %\pgfkeysgetvalue{/quantikz/gates/label style}{\labstyle}
  \pgfkeysgetvalue{/quantikz/gates/partial position}{\pos}
  \pgfkeysgetvalue{/quantikz/gates/label style}{\lstyle}
  \ifdefstring{\wtype}{c}{%
\edef\tempstyle{"{\partial}"{grade,pos=\pos,\lstyle,xshift=-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}},\tstyle}
  }{%
  \edef\tempstyle{"{\partial}"{grade,pos=\pos,\lstyle},\tstyle}
  }
%   \expandafter\expandedwire\expandafter{\tempstyle}{q}{d}{#2}
%   %\wire[d][#3][\tempstyle]{q}
  }
 \expandafter\expandafter\expandafter\expandedwire\expandafter\expandafter\expandafter{\expandafter\tempstyle\expandafter}\expandafter{\wtype}{d}{#2}
}



%misc
\DeclareDocumentCommand{\makeebit}{O{}m}{
  \pgfkeys{/quantikz/gates/.cd,style=,label style=,angle=-45,#1}%
  \pgfkeysgetvalue{/quantikz/gates/angle}{\angle}
  \pgfkeysgetvalue{/quantikz/gates/style}{\style}
  \pgfkeysgetvalue{/quantikz/gates/label style}{\lstyle}
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\make@ebit\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\style\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\lstyle\expandafter}\expandafter{\angle}{#2}
	%\arrow[arrows,line cap=round,\style,to path={(\tikztostart) -- ($(\tikztostart)!{0.5/cos(\angle)}!\angle:(\tikztotarget)$) node [anchor=east,style={\lstyle}]{#2} -- (\tikztotarget) }]{d}
}
\DeclareDocumentCommand{\make@ebit}{mmmm}{%
  \arrow[arrows,line cap=round,#1,to path={(\tikztostart) --  ($(\tikztostart)!{0.5/cos(#3)}!#3:(\tikztotarget)$) node [anchor=east,style={#2}]{#4} --(\tikztotarget) }]{d}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% helpers
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newlength{\myl}
\newlength{\myh}
\newlength{\myd}

%\makeatletter
\newcounter{aaa}
\tikzset{
  apply/.style args={#1 except on segments #2}{postaction={
      /utils/exec={
        \@for\mattempa:=#2\do{\csdef{aaa@\mattempa}{}}
        \setcounter{aaa}{0}
      },
      decorate,decoration={show path construction,
        moveto code={},
        lineto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path[#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
        curveto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..(\tikzinputsegmentlast);
          }
        },
        closepath code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
      },
    },
  },
}


%
%commands for putting in text vertically (e.g. for slices)
\protected\def\verticaltext#1{\leavevmode\bgroup\vbox\bgroup\xvvv#1\relax}
%
\def\xvvv{\afterassignment\xxvvv\let\tmp= }
%
\def\xxvvv{%
% \ifx\tmp\@sptoken\egroup\ \vbox\bgroup\let\next\xvvv
% \else
\ifx\tmp\relax\egroup\egroup\let\next\relax
 \else
\hbox to 1.1em{\hfill\tmp\hfill}% centred
\let\next\xvvv\fi%\fi
\next}
%end of commands for putting text vertically
%
\long\def\ifnodedefined#1#2#3{%
    \@ifundefined{pgf@sh@ns@#1}{#3}{#2}%
}

%find the vertical position of the middle of an equals sign
%https://tex.stackexchange.com/questions/355680/how-can-i-vertically-align-an-equals-sign-in-a-tikz-node/355686
\pgfmathsetmacro\MathAxis{height("$\vcenter{}$")}



\newcounter{wirenumberpermute}

\newcommand{\permute}[1]{%
\hphantom{Wide}%
\def\firstlist{#1}
 	\edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
 	\edef\mn{\the\numexpr\m-1\relax}
 	\edef\mp{\the\numexpr\m+1\relax}
 	\settowidth{\myl}{$Wide$}
 	\setcounter{wirenumberpermute}{0}
 	\foreach \x [count=\c] in \firstlist {%
 		\edef\start{\the\numexpr\c+\n-1\relax}%
 		\edef\endy{\the\numexpr\x+\n-1\relax}%
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
    \csxdef{cell@width@\start-\m}{\the\myl} %save the cell width for every row in a global variable
 		\stepcounter{wirenumberpermute}
 	 	}
 	 	\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter{%
 	 	\expandafter\expandafter\expandafter\wirepair@end\expandafter\expandafter\expandafter{\expandafter\n\expandafter}\expandafter{\m}{#1}%
 		}
 	\edef\lim{\the\numexpr\arabic{wirenumberpermute}+\n-1\relax}
 	 	\foreach \i in {\n,...,\lim} {%
 	     \edef\newcom{\noexpand\vqwexplicit{\i-\m}{\i-\mn}}
 	 		 \newcom%
 	 	}
}

\newcommand{\wirepair@end}[3]{%#row,col of left-most site. #row of right-most site.
	\xdef\LoopGG{}
	\edef\i{#1}
	\def\firstlist{#3}
	%\show\i
	%\show\j
	%create a list of cell names to be included in this grouped gate
	\foreach \n in \firstlist {%
	\ifnodedefined{\tikzcdmatrixname-\the\numexpr\n+\i-1\relax-#2}{%
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\the\numexpr\n+\i-1\relax-#2)}
		}{}
	}
	\ifnodedefined{\tikzcdmatrixname-\i-#2}{%
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\i-#2)}
		}{}
	\node (group\tikzcdmatrixname-#1-#2) [fit=\LoopGG,transparent,inner sep=0pt] {\phantom{Wide}};
		\foreach \n [count=\c] in \firstlist{%
			\draw [line width=3pt,\pgfkeysvalueof{/tikz/commutative diagrams/background color},shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-#1-#2.west|-\tikzcdmatrixname-\the\numexpr\i+\c-1\relax-#2.center) to[out=0,in=180] (group\tikzcdmatrixname-#1-#2.east|-\tikzcdmatrixname-\the\numexpr\i+\n-1\relax-#2.center);
			\draw [thickness] (group\tikzcdmatrixname-#1-#2.west|-\tikzcdmatrixname-\the\numexpr\i+\c-1\relax-#2.center) to[out=0,in=180] (group\tikzcdmatrixname-#1-#2.east|-\tikzcdmatrixname-\the\numexpr\i+\n-1\relax-#2.center);
		}
}


%%%
%
%the main gate command
%
%%%

\DeclareExpandableDocumentCommand{\gate}{O{}O{1.5pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner sep=4pt,minimum width=#2,minimum height=#3]|%
 	\edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
 	%reset macros that are going to be set by the options
 	\edef\options{row=\n,col=\m,#1}
 	\def\toswap{0}%
 	\def\DisableMinSize{0}%
 	%\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
 	%import options passed as parameters
  	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=,ps=,#1}%
 	\pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}%
  \ifnumless{\quantwires}{0}{%
    \PackageError{quantikz}{You cannot have a gate command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantwires}{0}{%
        \PackageError{quantikz}{You cannot have a gate command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
  \pgfkeyssetevalue{/quantikz/gates/style}{\pgfkeysvalueof{/quantikz/gates/ps},\pgfkeysvalueof{/quantikz/gates/style}}
 	\pgfkeysgetvalue{/quantikz/gates/style}{\a}%
 	\pgfkeysgetvalue{/quantikz/gates/label style}{\b}%
 	\ifthenelse{\toswap=1}{%if it's a swap gate...
  \ifnumequal{\quantwires}{2}{%good!
  }{%
  \PackageWarning{quantikz}{You have asked for a swap gate in cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn. This required the number of wires that the gate acts on to be overridden. Check this is your intended behaviour}
 		\pgfkeys{/quantikz/gates/wires=2}
 		\def\quantwires{2}
    }
 		\phantom{wide}
 		\settowidth{\myl}{$wide$}
 		\settoheight{\myh}{$wide$}
 		\settodepth{\myd}{$wide$}
 	}{%not a swap gate
  %figure out how large the per-cell box should be
 		\settowidth{\myl}{$#4$}
 		\ifthenelse{\DisableMinSize=1}{%disable automatic size detection. Use $U$ instead.
 			\phantom{U}
 			\settoheight{\myh}{$U$}
 			\settodepth{\myd}{$U$}
 		}{%automatically get width and height of label
 			\phantom{#4}
 			\settoheight{\myh}{$#4$}
 			\settodepth{\myd}{$#4$}
 		}
 	}
%	communicate per-cell sizes to the other cells
 	\edef\k{\the\numexpr\n+\quantwires-1\relax}
% 	\edef\mn{\the\numexpr\m-1\relax}
  \ifnumgreater{\quantwires}{1}{%
 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
    \csxdef{cell@width@\i-\m}{max(\the\myl+8pt,#2)} %save the cell width for every row in a global variable
 	}
  \csxdef{cell@height@\k-\m}{max(\the\myh+\the\myd+8pt,#3)} %apply auto height to last row only.
%		
 	}{}
 	%call deferred gate command. to be executed after the tikzcd matrix stuff is completed
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gate@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\a\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\b\expandafter}\expandafter{\options}{#4}
	}
}

%deferred gate command. draws a box around all included cells. this is not part of the matrix, but comes afterwards.
\newcommand{\gate@end}[4]{
	\pgfkeys{/quantikz/gates/.cd,wires=1,priority label={center}}
	\def\toswap{0}
	\def\DisableMinSize{0}
 	\pgfkeys{/quantikz/gates/.cd,#3}%import options
	\pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/gates/row}{\row}
	\pgfkeysgetvalue{/quantikz/gates/col}{\col}
  \pgfkeysgetvalue{/quantikz/gates/priority label}{\priority}
	\ifthenelse{\toswap=1}{\def\quantwires{2}}{}
	\xdef\LoopGG{}
	%create a list of cell names to be included in this grouped gate
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\n-\col)}
		}{}
	}
	\ifthenelse{\toswap=1}{%
		\node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,#1] {\hphantom{Wide}};
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\row-\col.center) to[out=0,in=180] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [line width=3pt,\pgfkeysvalueof{/tikz/commutative diagrams/background color},shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
	}{%
	%the actual gate drawing command
	  \node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,label={[gg label,#2]\priority:$#4$},#1] {\hphantom{$#4$}};
	}
}

%ghost will get height correct if can't be automatically assigned.
\DeclareExpandableDocumentCommand{\ghost}{O{0pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner ysep=4pt,minimum width=#1,minimum height=#2]| \vphantom{#3}
}

%%%
%
%slicing
%
%%%

%single slice
\newcommand\slice[2][]{%
	%\edef\currcol{\the\pgfmatrixcurrentcolumn}
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz/gates/.cd,#1}%
 	\edef\options{\pgfkeysvalueof{/quantikz/gates/style}}
 	\edef\opts{\pgfkeysvalueof{/quantikz/gates/label style}}
	\edef\n{\the\pgfmatrixcurrentcolumn}
	%\expandafter\show\n
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendslices\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}}
%deferred slice command
\newcommand{\slice@end}[4]{
	\edef\top{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row1.north)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row1.north)$)}
	\edef\bottom{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+(0,-3pt)$)}
	\expandafter\expandafter\expandafter\make@slice\expandafter\expandafter\expandafter{\expandafter\top\expandafter}\expandafter{\bottom}{#4}{#2}{#3}
}
\newcommand{\make@slice}[5]{
	\draw[slice,#4] #1 to node[pos=0,inner sep=4pt,anchor=south,color=black,#5] {#3} #2;
}
%deferred command which will slice everything
\newcommand{\sliceallr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/commutative diagrams/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/commutative diagrams/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/commutative diagrams/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\pgfkeysvalueof{/tikz/commutative diagrams/slice titles}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}
%deferred slice command with vertical text
\newcommand{\sliceallvr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/commutative diagrams/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/commutative diagrams/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/commutative diagrams/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\verticaltext{\pgfkeysvalueof{/tikz/commutative diagrams/slice titles}}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}

%labelling of inputs
\newcommand\lstick[2][]{%
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz/gates/.cd,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/gates/label style}{\options}
	\pgfkeysgetvalue{/quantikz/gates/braces}{\opts}
  \pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}
   \ifnumless{\quantwires}{0}{%
    \PackageError{quantikz}{You cannot have an lstick command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantwires}{0}{%
        \PackageError{quantikz}{You cannot have an lstick command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupinput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%labelling of outputs
\newcommand\rstick[2][]{%
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz/gates/.cd,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/gates/label style}{\options}
	\pgfkeysgetvalue{/quantikz/gates/braces}{\opts}
    \pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}
   \ifnumless{\quantwires}{0}{%
    \PackageError{quantikz}{You cannot have an rstick command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantwires}{0}{%
        \PackageError{quantikz}{You cannot have an rstick command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}

\newcommand\midstick[2][]{%
	\hphantom{\text{g#2g}}\ %leave enough space for whatever text we've inserted
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz/gates/.cd,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/gates/label style}{\options}
	\pgfkeysgetvalue{/quantikz/gates/braces}{\opts}
   \ifnumless{\quantwires}{0}{%
    \PackageError{quantikz}{You cannot have a midstick command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantwires}{0}{%
        \PackageError{quantikz}{You cannot have a midstick command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
	 \edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
	\edef\k{\the\numexpr\n+\quantwires-1\relax}
	\settowidth{\myl}{g#2g}
	%if more than 1 wire, need to reserve space for each wire
	\ifthenelse{\quantwires=1}{}{
	 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
    \csxdef{cell@width@\i-\m}{\the\myl} %save the cell width for every row in a global variable
 	}
%		
 	}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@mid\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
\newcommand{\ifcsstringeitheror}[4]{%
\ifcsstring{#1}{#2}{#4}{\ifcsstring{#1}{#3}{#4}{}}
}
%deferred labelling of inputs
\newcommand{\groupinput@end}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz/gates/.cd,wires=1}
	\def\rightbrace{1}
 	\pgfkeys{/quantikz/gates/.cd,#1}%
	\pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/gates/row}{\row}
	\pgfkeysgetvalue{/quantikz/gates/col}{\col}
	\xdef\LoopGI{}
  \ifcsstringeitheror{wire@type@\row}{c}{b}{%is the first wire classical? (should include bundle as well)
\xdef\LoopGI{\LoopGI($(\tikzcdmatrixname-\row-\col.center)+(0,\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})$)}
  }
   \ifcsstringeitheror{wire@type@\the\numexpr\row+\quantwires-1\relax}{c}{b}{%is the last wire classical? (should include bundle as well)
\xdef\LoopGI{\LoopGI($(\tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.center)+(0,-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})$)}
  }
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGI{\LoopGI(\tikzcdmatrixname-\n-\col)} 
		}{}
		}
	\ifthenelse{\quantwires=1} {
		\node (ingr-\row) [fit=\LoopGI, inner sep=0pt,label={[align=center,#2]left:#4}] {};
	}{
	\node (ingr-\row) [fit=\LoopGI, inner sep=0pt,label={[align=center,anchor=east,xshift=-0.2cm,#2]left:#4}] {};
	\ifthenelse{\rightbrace=1}{
	\draw[dm,#3] ($(ingr-\row.north west)+(-0.1cm,0.1cm)$) to ($(ingr-\row.south west)+(-0.1cm,-0.1cm)$);
	}{}
	}
} %
%deferred labelling of outputs
\newcommand{\groupoutput@end}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz/gates/.cd,wires=1}
	\def\leftbrace{1}
 	\pgfkeys{/quantikz/gates/.cd,#1}%
	\pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/gates/row}{\row}
	\pgfkeysgetvalue{/quantikz/gates/col}{\col}
	\xdef\LoopGO{}
    \ifcsstringeitheror{wire@type@\row}{c}{b}{%is the first wire classical? (should include bundle as well)
\xdef\LoopGO{\LoopGO($(\tikzcdmatrixname-\row-\col.center)+(0,\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})$)}
  }
   \ifcsstringeitheror{wire@type@\the\numexpr\row+\quantwires-1\relax}{c}{b}{%is the last wire classical? (should include bundle as well)
\xdef\LoopGO{\LoopGO($(\tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.center)+(0,-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})$)}
  }
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (outgr-\row) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]right:#4}] {};
	}{
	\node (outgr-\row) [fit=\LoopGO, inner sep=0pt,label={[align=center,anchor=west,xshift=0.2cm,#2]left:#4}] {};
	\ifthenelse{\leftbrace=1}{
	\draw[dd,#3] ($(outgr-\row.north east)+(0.1cm,0.1cm)$) to ($(outgr-\row.south east)+(0.1cm,-0.1cm)$);
	}{}
	}
} %
%deferred labelling in the middle of circuits
\newcommand{\groupoutput@mid}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz/gates/.cd,wires=1}
	\def\leftbrace{1}\def\rightbrace{1}
 	\pgfkeys{/quantikz/gates/.cd,#1}%
	\pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/gates/row}{\row}
	\pgfkeysgetvalue{/quantikz/gates/col}{\col}
	\xdef\LoopGO{}
    \ifcsstringeitheror{wire@type@\row}{c}{b}{%is the first wire classical? (should include bundle as well)
\xdef\LoopGO{\LoopGO($(\tikzcdmatrixname-\row-\col.center)+(0,\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})$)}
  }
   \ifcsstringeitheror{wire@type@\the\numexpr\row+\quantwires-1\relax}{c}{b}{%is the first wire classical? (should include bundle as well)
\xdef\LoopGO{\LoopGO($(\tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.center)+(0,-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap})$)}
  }
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		%\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]#4}] {};
		\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[align=center,anchor=mid,#2]center:#4}] {};
	}{
	\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[align=center,anchor=mid,#2]center:#4}] {};
	\ifthenelse{\rightbrace=1}{
	\draw[dm,#3] ($(midgr-\row-\col.north east)+(-0.1cm,0.05cm)$) to ($(midgr-\row-\col.south east)+(-0.1cm,-0.05cm)$);
	}{}
	\ifthenelse{\leftbrace=1}{
	\draw[dd,#3] ($(midgr-\row-\col.north west)+(0.1cm,0.05cm)$) to ($(midgr-\row-\col.south west)+(0.1cm,-0.05cm)$);
	}{}
	}
} %
%inputs and outputs within a multi-wire gate
\newcommand\gateinput[2][]{%
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=}%
	\pgfkeys{/quantikz/gates/.cd,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/gates/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/gates/braces}{\opts}%
    \pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}
   \ifnumless{\quantwires}{0}{%
    \PackageError{quantikz}{You cannot have a gate input command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantwires}{0}{%
        \PackageError{quantikz}{You cannot have a gate input command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mginput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
\newcommand\gateoutput[2][]{%
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz/gates/.cd,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/gates/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/gates/braces}{\opts}
    \pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}
   \ifnumless{\quantwires}{0}{%
    \PackageError{quantikz}{You cannot have a gate output command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantwires}{0}{%
        \PackageError{quantikz}{You cannot have a gate output command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mgoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred functions for the above
\newcommand{\mginput@end}[4]{%collected options,label style, brace style,text
	\pgfkeys{/quantikz/gates/.cd,wires=1}
 	\pgfkeys{/quantikz/gates/.cd,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/gates/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/gates/row}{\row}
	\pgfkeysgetvalue{/quantikz/gates/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0,0cm)$)[leftinternal,#2]{#4};
}{%
%\show\quantwires
\draw[dd,#3] ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0.1cm,0.1cm)$) to node[leftinternal,midway,#2] {#4} ($(\cell.west |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.west)+(0.1cm,-0.1cm)$);
}
} %
\newcommand{\mgoutput@end}[4]{%
	\pgfkeys{/quantikz/gates/.cd,wires=1}
 	\pgfkeys{/quantikz/gates/.cd,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/gates/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/gates/row}{\row}
	\pgfkeysgetvalue{/quantikz/gates/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(0,0cm)$)[rightinternal,#2]{#4};
}{%
\draw[dm,#3] ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(-0.1cm,0.1cm)$) to node[rightinternal,midway,#2] {#4} ($(\cell.east |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.east)+(-0.1cm,-0.1cm)$);
}
} %

%wave command
\newcommand\wave[1][]{%
\setwiretype{n}
	\edef\n{\the\pgfmatrixcurrentrow}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendslices\expandafter{%
		\expandafter\wave@end\expandafter{\n}{#1}%
	}
}
%deferred wave
\newcommand{\wave@end}[2]{
	\node (wave-#1) [fit=(\tikzcdmatrixname-row#1),wave,#2] {};
}


%put a border around a group of gates
\newcommand\gategroup[2][]{%
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=,steps=1}
	\pgfkeys{/quantikz/gates/.cd,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/gates/style}{\options}
 	\pgfkeysgetvalue{/quantikz/gates/label style}{\opts}
    \pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}
   \ifnumless{\quantwires}{0}{%
    \PackageError{quantikz}{You cannot have a gate group command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantwires}{0}{%
        \PackageError{quantikz}{You cannot have a gate group command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
    \pgfkeysgetvalue{/quantikz/gates/steps}{\steps}
   \ifnumless{\steps}{0}{%
    \PackageError{quantikz}{You cannot have a gate group command with a negative number of steps. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\steps}{0}{%
        \PackageError{quantikz}{You cannot have a gate group command with 0 steps. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gategroup@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred gate group command
\newcommand{\gategroup@end}[4]{%options, gate style, text style, text
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=,steps=1}%
	\edef\background{0}%
	\pgfkeys{/quantikz/gates/.cd,#1}%
	\pgfkeysgetvalue{/quantikz/gates/wires}{\quantwires}%
	\pgfkeysgetvalue{/quantikz/gates/row}{\row}%
	\pgfkeysgetvalue{/quantikz/gates/col}{\col}%
	\pgfkeysgetvalue{/quantikz/gates/steps}{\steps}%
	\edef\fit{(\tikzcdmatrixname-col\col.west |- \tikzcdmatrixname-row\row.north)(\tikzcdmatrixname-col\the\numexpr\col+\steps-1\relax.east |- \tikzcdmatrixname-row\the\numexpr\row+\quantwires-1\relax.south)}%
	\ifthenelse{\background=1}{%
		\begin{pgfonlayer}{background}\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};\end{pgfonlayer}
	}{%
		\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};
	}
}



% \newcommand{\latephase@end}[1]{
% 	\node [phase,inner sep=2pt] at (\tikzcdmatrixname-#1) {};
% }


%\makeatother

%this command runs after we've finished the matrix, and makes unified cells for each row and each column. This allows much nicer alignment of large boxes.
\newcommand{\DivideRowsCols}{
	\foreach \n in {1,...,\the\pgfmatrixcurrentrow} {%for each row, construct a master cell that contains all entries
	\xdef\LoopRow{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentcolumn}{
			\ifnodedefined{\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(\tikzcdmatrixname-\n-\m)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(group\tikzcdmatrixname-\n-\m)}
			}{}
	}
	\node (\tikzcdmatrixname-row\n) [fit=\LoopRow] {};
	}
	\foreach \n in {1,...,\the\pgfmatrixcurrentcolumn} {%for each column, construct a master cell that contains all entries
	\xdef\LoopCol{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentrow}{
			\ifnodedefined{\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(\tikzcdmatrixname-\m-\n)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(group\tikzcdmatrixname-\m-\n)}
			}{}
	}
	\node (\tikzcdmatrixname-col\n) [fit=\LoopCol] {};
	}
}

%this is the command that implements the align equals at key.
%take a parameter, row number, where we want to set the baseline. if not integer, use the two rows spanned
\providecommand{\setmiddle}[1]{%
\IfInteger{#1}{
\pgfmathtruncatemacro\wholepart{floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]\noexpand\tikzcdmatrixname-\wholepart-1.center)}
}}
%\show\temp
\temp
}{%
\pgfmathtruncatemacro\wholepart{floor(#1)}
\pgfmathtruncatemacro\neighbour{floor(#1)+1}
\pgfmathsetmacro\fractionalpart{#1-floor(#1)}
\edef\temp{
%\noexpand\tikzset{every matrix/.append style={baseline=([yshift=-\MathAxis]$(\noexpand\tikzcdmatrixname-\wholepart-1.base)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.base)$)}%
\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]$(\noexpand\tikzcdmatrixname-\wholepart-1.center)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.center)$)}
}}
%\show\temp
\temp
}
}

% \providecommand{\setmiddle}[1]{%
% \IfInteger{#1}{
% \pgfmathtruncatemacro\wholepart{floor(#1)}
% \edef\temp{\noexpand\tikzset{%
% /tikz/baseline={(\noexpand\tikzcdmatrixname-\wholepart-1.base)}
% }}
% %\show\temp
% \temp
% }{%
% \pgfmathtruncatemacro\wholepart{floor(#1)}
% \pgfmathtruncatemacro\neighbour{floor(#1)+1}
% \pgfmathsetmacro\fractionalpart{#1-floor(#1)}
% \edef\temp{
% %\noexpand\tikzset{every matrix/.append style={baseline=([yshift=-\MathAxis]$(\noexpand\tikzcdmatrixname-\wholepart-1.base)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.base)$)}%
% \noexpand\tikzset{%
% /tikz/baseline={($(\noexpand\tikzcdmatrixname-\wholepart-1.base)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.base)$)}
% }}
% %\show\temp
% \temp
% }
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Option parameter processing via key/value pairs
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%initialise all the pgfkeys for key=value parameter passing in macro options
\tikzcdset{%
	slice all/.code={\gdef\toslice@qtkz{1}},
	remove end slices/.initial=0,
	slice titles/.initial={\col},
	slice style/.initial={},
	slice label style/.initial={},
	thin lines/.code={\resetstyles},
	transparent/.code={\maketransparent},
	vertical slice labels/.code={\def\vert@qtkz{1}},
	align equals at/.code={\setmiddle{#1}},
  wire types/.code={\importwiretypes{#1}},
  classical gap/.initial=0.03cm, % define separation of classical wires (can override)
 % wire style/.code={\gdef\quantikzopts{#1}},
}
\pgfkeys{/quantikz/gates/.cd,%
	.unknown/.style={%
		/quantikz/gates/wires=\pgfkeyscurrentname
	},%
	%wires/.store in=\quantwires,%
	wires/.initial=1,%
	style/.initial={},
	label style/.initial={},
	braces/.initial={},
	background/.code={\def\background{1}},
	%alternate/.default=1,
	%alternate/.code={\def\helper{#1}},
  alternate/.code={\PackageWarning{quantikz}{Use of alternate is deprecated.}},
	row/.initial=1,
	col/.initial=1,
	steps/.initial=1,
	Strike Width/.initial=0.08cm,
	Strike Height/.initial=0.12cm,
	swap/.code={\def\toswap{1}},
	disable auto height/.code={\def\DisableMinSize{1}},
  nwires/.code={\PackageWarning{quantikz}{Use of nwires is deprecated. Set wire types globally instead.}},
  cwires/.code={\PackageWarning{quantikz}{Use of cwires is deprecated. Set wire types globally instead.}},
	brackets/.is choice,
	brackets/.initial=both,
  priority label/.initial={},
  ps/.initial={},
  angle/.initial=-45,
  vertical wire/.initial=q,
  wire style/.initial={},
  open/.code={\tikzset{filling}},
  partial swap/.initial={},
  partial position/.initial={0.5},
}
\pgfkeys{/quantikz/gates/brackets/.cd,%define brackets options
	none/.code={\def\leftbrace{0}\def\rightbrace{0}},
	left/.code={\def\leftbrace{1}\def\rightbrace{0}},
	right/.code={\def\leftbrace{0}\def\rightbrace{1}},
	both/.code={\def\leftbrace{1}\def\rightbrace{1}}
}
% \pgfkeys{/quantikz/swap/.cd,%define options for swap gate
%   partial/.initial={},
%   position/.initial={0.5},
%   label style/.initial={}
% }


%my standard Dirac notation commands. can be overridden by user.
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right |}}
\providecommand{\proj}[1]{\ensuremath{\ket{#1}\!\bra{#1}}}
\providecommand{\braket}[2]{\ensuremath{\left\langle#1\middle|#2\right\rangle}}
\newcommand{\forceredefine}{%
\renewcommand{\ket}[1]{\ensuremath{\left|##1\right\rangle}}
\renewcommand{\bra}[1]{\ensuremath{\left\langle##1\right |}}
\renewcommand{\proj}[1]{\ensuremath{\ket{##1}\!\bra{##1}}}
\renewcommand{\braket}[2]{\ensuremath{\left\langle##1\middle|##2\right\rangle}}
}


%\DeclareExpandableDocumentCommand{\ctrlbundle}{O{1}O{}m}{|[phase bundle,#2]| {} \vqw{#3}\qwbundle[alternate=#1]{}}

%wire commands with absolute positioning. Need updating.
\newcommand{\vqwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {}
}
% \newcommand{\vqbundleexplicit}[2]{
% 	\arrow[from=#1,to=#2,arrows] {} \arrow[from=#1,to=#2,arrows,yshift=0.1cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.1cm] {}
% }
% %classical vertical wire, absolute positioning
% \newcommand{\vcwexplicit}[2]{
% 	\arrow[from=#1,to=#2,arrows,xshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,xshift=-0.05cm] {}
% }
% %classical horizontal wire, absolute positioning
% \newcommand{\vcwhexplicit}[2]{
% 	\arrow[from=#1,to=#2,arrows,yshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.05cm] {}
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Style properties
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%configure some of the style properties.
%annoyingly, this first one will affect all tikzcd instances, not just quantum circuits. I should have only provided the quantikz environment as a modified version of tikzcd, and not allowed direct use of tikzcd. Probably too late now.
\tikzcdset{%
	row sep/normal=0.5cm,
	column sep/normal=0.5cm,
	thick,
	nodes in empty cells,
	every cell/.style={
        anchor=center,minimum size=0pt,inner sep=0pt,outer sep=0pt,thick,
        minimum height=\ifcsundef{cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}{0}{\csname cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn\endcsname},
        minimum width=\ifcsundef{cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}{0}{\csname cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn\endcsname},
        %append after command={\wire{a}}
        execute at end cell={\wire{a}%looks promising. does not work on empty cells.
        %be careful to unset "global" variables that really only apply to current diagram
        \csgundef{cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      \csgundef{cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      \csgundef{wire@type@override@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}}
    },
  arrows/.style={dash,thick,line cap=round},
  %1-row diagram/.style={},
  1-row diagram/.style={/tikz/baseline={([yshift=-\MathAxis]\tikzcdmatrixname-1-1.center)}},%doesn't seem to be doing anything. Possibly activates too late?
  grade/.style={description,circle,draw,fill=white,inner sep=0pt, outer sep=0pt,font=\tiny}
}
\tikzset{
	thickness/.style={thick},
  filling/.style={fill=\pgfkeysvalueof{/tikz/commutative diagrams/background color}},
  operator/.style={draw,filling, inner sep=2pt,thickness,align=center},
  ggroup/.style={draw,minimum size=1.5em,thickness,align=center,inner sep=4pt},
  leftinternal/.style={anchor=mid west,font=\scriptsize,inner sep=4pt,align=center},
  rightinternal/.style={anchor=mid east,font=\scriptsize,inner sep=4pt,align=center},
  wave/.style={inner sep=-3pt,tape,filling,apply={draw=black} except on segments {5,6,1,2,9}},
  phase bundle/.style={fill,shape=rectangle,rounded corners=1.5pt,minimum width=4pt,minimum height=10pt},
  internal/.style={thickness},
 %  rectangle with rounded corners north west/.initial=0pt,
	% rectangle with rounded corners south west/.initial=0pt,
	% rectangle with rounded corners north east/.initial=8pt,
	% rectangle with rounded corners south east/.initial=8pt,
  line/.style={path picture={ 
		\draw[internal](path picture bounding box.west) -- (path picture bounding box.east);
	}},
	%hidden bend/.style={path picture={
%		\draw[internal,inner sep=0pt] (path picture bounding box.west) -- (path picture bounding box.center) -- (path picture bounding box.south);},
%		minimum height=1.5em,minimum width=1em},
  dd/.style={decoration={brace},decorate,thickness},
  dm/.style={decoration={brace,mirror},decorate,thickness},
  slice/.style={thickness,red,dash pattern=on 5pt off 3pt,align=center},
 	my labelcw/.style={yshift=0.04cm,above,align=center},
 	gg label/.style={label position=center,align=center},
 	group label/.style={label position=above,yshift=0.2cm,anchor=mid}
}

\def\resetstyles{
\tikzcdset{thin,every cell/.append style={thin},arrows/.append style={thin}
    }
\tikzset{
	thickness/.style={thin},
	%operator/.append style={thin},
	%internal/.append style={thin},
	%dd/.append style={thin},
	%dm/.append style={thin},
	%slice/.append style={thin},
	meter/.append style={thin},
	phase/.append style={minimum size=3pt},
%	ophase/.append style={minimum size=3pt},
	%circlewc/.append style={minimum size=3pt,inner sep=2pt}
}
}

\def\maketransparent{
\tikzset{
  filling/.append style={fill opacity=0,text opacity=1},
%	operator/.append style={fill opacity=0},
	% meter/.append style={fill opacity=0},
	% measuretab/.append style={fill opacity=0},
	% meterD/.append style={fill opacity=0},
	% measure/.append style={fill opacity=0},
	% wave/.append style={fill opacity=0},
%	ophase/.append style={fill opacity=0}
}
}

